Continual World: A Robotic Benchmark For Continual Reinforcement Learning

Continual learning (CL) -- the ability to continuously learn, building on previously acquired knowledge -- is a natural requirement for long-lived autonomous reinforcement learning (RL) agents. While building such agents, one needs to balance opposing desiderata, such as constraints on capacity and compute, the ability to not catastrophically forget, and to exhibit positive transfer on new tasks. Understanding the right trade-off is conceptually and computationally challenging, which we argue has led the community to overly focus on catastrophic forgetting. In response to these issues, we advocate for the need to prioritize forward transfer and propose Continual World, a benchmark consisting of realistic and meaningfully diverse robotic tasks built on top of Meta-World as a testbed. Following an in-depth empirical evaluation of existing CL methods, we pinpoint their limitations and highlight unique algorithmic challenges in the RL setting. Our benchmark aims to provide a meaningful and computationally inexpensive challenge for the community and thus help better understand the performance of existing and future solutions. Information about the benchmark, including the open-source code, is available at https://sites.google.com/view/continualworld.

==> 609bc59dc39be977132478d8 copy/ablations.tex <==
\subsection{Other orders of tasks}
\label{app:abl_order}
We study the impact of task order on the performance of CL methods. In Figure~\ref{fig:abl_order}, we show average performance curves for three selected CL methods that are run with the same hyperparameters on three different orderings: the  CW10 sequence (see Section \ref{sec:sequences_appendix}) and its two random permutations.
Further, Table~\ref{tab:ablation_order} contains values of the forgetting and forward transfer metrics.

The ranking of the methods is preserved; we also observe that forward transfer of EWC varies substantially with the change of sequence order. To a lesser extent, this also impacts the performance metric. Decreasing this variance is, in our view, an important research question. We speculate that it is much related to improving transfer in general. 

\begin{table}[ht!]
    \begin{center}
        \tabcolsep=0.11cm
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}{llll}
            \toprule
            method                                      & performance               & forgetting                 & f. transfer                  \\
            \midrule
            \textbf{Fine-tuning, CW10 order (standard)} & 0.10 {\tiny [0.10, 0.11]} & 0.74 {\tiny [0.72, 0.75]}  & 0.32 {\tiny [0.29, 0.35]}    \\
            \textbf{EWC, CW10 order (standard)}         & 0.66 {\tiny [0.63, 0.69]} & 0.03 {\tiny [0.01, 0.06]}  & 0.02 {\tiny [-0.05, 0.07]}   \\
            \textbf{PackNet, CW10 order (standard)}     & 0.87 {\tiny [0.85, 0.89]} & 0.01 {\tiny [-0.01, 0.02]} & 0.38 {\tiny [0.36, 0.41]}    \\
            \midrule
            \textbf{Fine-tuning, CW10 permutation 1}    & 0.10 {\tiny [0.10, 0.10]} & 0.72 {\tiny [0.69, 0.74]}  & 0.18 {\tiny [0.13, 0.23]}    \\
            \textbf{EWC, CW10 permutation 1}            & 0.46 {\tiny [0.43, 0.50]} & 0.02 {\tiny [0.00, 0.04]}  & -0.45 {\tiny [-0.50, -0.41]} \\
            \textbf{PackNet, CW10 permutation 1}        & 0.82 {\tiny [0.80, 0.84]} & 0.03 {\tiny [0.01, 0.05]}  & 0.25 {\tiny [0.19, 0.30]}    \\
            \midrule
            \textbf{Fine-tuning, CW10 permutation 2}    & 0.10 {\tiny [0.10, 0.10]} & 0.73 {\tiny [0.72, 0.75]}  & 0.22 {\tiny [0.19, 0.26]}    \\
            \textbf{EWC, CW10 permutation 2}            & 0.48 {\tiny [0.43, 0.52]} & 0.05 {\tiny [0.03, 0.07]}  & -0.54 {\tiny [-0.68, -0.42]} \\
            \textbf{PackNet, CW10 permutation 2}        & 0.84 {\tiny [0.81, 0.86]} & 0.01 {\tiny [0.00, 0.03]}  & 0.30 {\tiny [0.26, 0.34]}    \\
            \bottomrule
        \end{tabular}
        \caption{Results on the CW10 sequence and its 2 random permutations.}
        \label{tab:ablation_order}
    \end{center}
\end{table}

\begin{figure}[h!]
    \begin{center}
        % \includegraphics[width=\textwidth]{imgs/abl_order_1.png}
        % \includegraphics[width=\textwidth]{imgs/abl_order_2.png}
        % \includegraphics[width=\textwidth]{imgs/abl_order_3.png}
        \includegraphics[width=\textwidth]{imgs/abl_order_merged.png}
        \caption{\label{fig:abl_order} Average performance for selected methods on CW10 and its two random orderings.}
    \end{center}
\end{figure}

The new sequences are:

{\small
\texttt{handle-press-side-v1, faucet-close-v1, shelf-place-v1,  stick-pull-v1, peg-unplug-side-v1, hammer-v1, push-back-v1, push-wall-v1, push-v1, window-close-v1}}

and

    {\small \texttt{stick-pull-v1, push-wall-v1, shelf-place-v1,
            window-close-v1, hammer-v1, peg-unplug-side-v1,
            push-back-v1, faucet-close-v1, push-v1,
            handle-press-side-v1.}}


\subsection{Random order of tasks}\label{subsec:random_orders}

We further study the impact of task orderings by evaluating on $20$ different random orders, see Table~\ref{tab:random_orders}. Obtained results are qualitatively similar to the ones with the fixed ordering.

%We generate 20 random permutations of CW10.
% In  we report results for all the methods. Each metric is computed as an average over 20 different random orders of CW10.

\begin{table}[ht!]
    \begin{center}
        \tabcolsep=0.11cm
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}{llll}
\toprule
 method   & performance       & forgetting          & f. transfer   \\
\midrule
 \textbf{Fine-tuning}        & 0.08 {\tiny [0.07, 0.09]} & 0.71 {\tiny [0.68, 0.74]}   & 0.17 {\tiny [0.09, 0.24]}     \\
 \textbf{L2}          & 0.42 {\tiny [0.34, 0.49]} & 0.00 {\tiny [-0.01, 0.01]}  & -0.73 {\tiny [-0.90, -0.56]}  \\
 \textbf{EWC}         & 0.53 {\tiny [0.48, 0.58]} & 0.01 {\tiny [-0.01, 0.03]}  & -0.31 {\tiny [-0.43, -0.18]}  \\
 \textbf{MAS}         & 0.41 {\tiny [0.35, 0.47]} & 0.00 {\tiny [-0.02, 0.02]}  & -0.65 {\tiny [-0.79, -0.51]}  \\
 \textbf{VCL}         & 0.39 {\tiny [0.34, 0.44]} & 0.02 {\tiny [-0.00, 0.03]}  & -0.69 {\tiny [-0.80, -0.58]}  \\
 \textbf{PackNet}     & 0.72 {\tiny [0.68, 0.76]} & 0.00 {\tiny [-0.01, 0.01]}  & -0.04 {\tiny [-0.14, 0.05]}   \\
 \textbf{Perfect Memory}   & 0.27 {\tiny [0.24, 0.31]} & -0.00 {\tiny [-0.02, 0.01]} & -1.12 {\tiny [-1.22, -1.02]}  \\
 \textbf{A-GEM}        & 0.10 {\tiny [0.08, 0.11]} & 0.70 {\tiny [0.67, 0.73]}   & 0.19 {\tiny [0.12, 0.24]}     \\
\bottomrule
\end{tabular}
        \caption{Results averaged over 20 different random orderings of CW10 -- see Subsection~\ref{subsec:random_orders}}
        \label{tab:random_orders}
    \end{center}
\end{table}

\subsection{One-hot inputs}
We study an alternative setup in which a single-head architecture is used, and one-hot encoding is provided in input for the task identification. In Table \ref{tab:ablation_sh} and Figure~\ref{fig:abl_sh} we present results for three selected CL methods in both the multi-head and single-head setups. We see that the performance of EWC drops a bit, while PackNet remains mostly unaffected. Table~\ref{tab:ablation_sh} contains values of average performance, forgetting, and forward transfer computed in this setting.

For the single-head experiments, we ran another hyperparameter search. For the single-head EWC experiment the selected value is $\lambda = 10^3$ as opposed to $\lambda = 10^4$ for multi-head. We conjecture that the multi-head case can be regularized more aggressively, as for each task, it gets a small number of new parameters (in new heads).

\begin{figure}
    \begin{center}
        \includegraphics[width=\textwidth]{imgs/abl_sh_merged.png}
        \caption{\label{fig:abl_sh} Average performance for selected CL methods on CW10 with standard multi-head architecture and single-head architecture with one-hot task encoding added to input.}
    \end{center}
\end{figure}


\begin{table}[ht!]
    \begin{center}
        \tabcolsep=0.11cm
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}{llll}
            \begin{tabular}{llll}
                \toprule
                method                                       & performance               & forgetting                  & f. transfer                  \\
                \midrule
                \textbf{Fine-tuning, Multi-head (standard) } & 0.10 {\tiny [0.10, 0.11]} & 0.74 {\tiny [0.72, 0.75]}   & 0.32 {\tiny [0.29, 0.35]}    \\
                \textbf{EWC, Multi-head (standard)}          & 0.66 {\tiny [0.63, 0.69]} & 0.03 {\tiny [0.01, 0.06]}   & 0.02 {\tiny [-0.05, 0.07]}   \\
                \textbf{PackNet, Multi-head (standard)}      & 0.87 {\tiny [0.85, 0.89]} & 0.01 {\tiny [-0.01, 0.02]}  & 0.38 {\tiny [0.36, 0.41]}    \\
                \midrule
                \textbf{Fine-tuning, Single-head + one-hot } & 0.12 {\tiny [0.12, 0.13]} & 0.68 {\tiny [0.66, 0.70]}   & 0.16 {\tiny [0.12, 0.19]}    \\
                \textbf{EWC, Single-head + one-hot}          & 0.48 {\tiny [0.45, 0.50]} & 0.14 {\tiny [0.12, 0.15]}   & -0.25 {\tiny [-0.33, -0.17]} \\
                \textbf{PackNet, Single-head + one-hot}      & 0.87 {\tiny [0.85, 0.89]} & -0.01 {\tiny [-0.02, 0.01]} & 0.24 {\tiny [0.20, 0.28]}    \\
                \bottomrule
            \end{tabular}
        \end{tabular}
        \caption{Results on CW10 with original multi-head setup and alternative with single-head and one-hot encoding}
        \label{tab:ablation_sh}
    \end{center}
\end{table}

\label{sec:onehot}

\subsection{Experiments with a sequence of $30$ tasks}

An important question for continual learning is how methods scale to a larger number of tasks. To test this in our setting, we consider a sequence of $30$ tasks. To select challenging but solvable tasks we removed $10$ easiest and $10$ hardest task of MetaWorld (measured by performance in single-task learning). 


% An intriguing question in continual learning is how methods scale to a larger number of tasks. To test this in our setting, we consider a sequence of $30$ tasks. The sequence is obtained by taking the base $50$ tasks from MetaWorld and removing $10$ easiest and $10$ hardest tasks, as measured by performance of a single-task learner. This is done in order to avoid training on tasks which are either nearly impossible or trivial to learn, which allows us to focus on tasks which are challenging, but still solvable.

This way we obtained a set of $30$ following tasks:
{\small \textsc{plate-slide-v1}, \textsc{plate-slide-back-side-v1}, \textsc{handle-press-v1}, \textsc{handle-pull-v1}, \textsc{handle-pull-side-v1}, \textsc{soccer-v1}, \textsc{coffee-push-v1}, \textsc{coffee-button-v1}, \textsc{sweep-into-v1}, \textsc{dial-turn-v1}, \textsc{hand-insert-v1}, \textsc{window-open-v1}, \textsc{plate-slide-side-v1}, \textsc{plate-slide-back-v1}, \textsc{door-lock-v1}, \textsc{door-unlock-v1}, \textsc{push-v1}, \textsc{door-open-v1}, \textsc{box-close-v1}, \textsc{faucet-open-v1}, \textsc{coffee-pull-v1}, \textsc{shelf-place-v1}, \textsc{faucet-close-v1}, \textsc{handle-press-side-v1}, \textsc{push-wall-v1}, \textsc{sweep-v1}, \textsc{stick-push-v1}, \textsc{bin-picking-v1}, \textsc{basketball-v1}, \textsc{hammer-v1}}.


We then train four methods: fine-tuning, EWC, PackNet, and Perfect Memory on this set of tasks. We use the random ordering approach presented in Subsection \ref{subsec:random_orders} with 40 seeds to obtain reliable results. The tested methods perform similarly as in the case of CW20, see Table \ref{tab:ablation_cw30}.  PackNet significantly outperforms the rest of the methods, followed by EWC. Reservoir and fine-tuning are affected with catastrophic forgetting, with performance showing that they are mostly able to solve a single task. %Since the base setup of $20$ tasks shows similar findings with reduced computational complexity, we decide to use this setting as our main one.

\begin{table}[ht!]
    \begin{center}
        \begin{tabular}{crrrr}
            \toprule
               & Fine-tuning   & EWC & PackNet & Perfect Memory  \\
            \midrule%\small 
            \textbf{Performance} & 0.04 {\small [0.03, 0.04]} & 0.44 {\small [0.42, 0.46]}   & 0.70 {\small [0.68, 0.71]} & 0.04 {\small [0.03, 0.04]} \\
            \bottomrule
        \end{tabular}
        \caption{Results on 30 tasks.}
        \label{tab:ablation_cw30}
    \end{center}
\end{table}

==> 609bc59dc39be977132478d8 copy/cl_challenges.tex <==
% \piotrm{Change the title. Any suggestions?} "Adaptations to CL setting ???"

This section lists various challenges that we encountered while implementing the CL methods described in Section \ref{sec:cl_methods_appendix}. In most cases, they stem from the fact that the methods were initially developed for supervised learning and needed to be adopted to the more algorithmically complex RL setting.


\subsection{Critic regularization} \label{sec:critic_regularizaiton_appendix}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/appendix/ewc_critic_ablation.png}
    \caption{Average performance for EWC with various settings of the critic regularization, see \eqref{eq:generic_regularization}. The reference dashed lines show the performance without critic regularization.}
    \label{fig:ewc_critic_ablation_appendix}
\end{figure}

One of perhaps most important algorithmic conclusions is that \emph{regularizing the critic network is harmful to performance}. We recall that in all methods, except for AGEM and Perfect Memory, the critic is only used during the training. Consequently, it needs to store only the value function for the current task, and thus forgetting is not a (primary) issue. Further, one can opt for not using any CL method on the critic network. The rationale for such a decision is to maintain the full network ``plasticity'' (which is typically reduced by CL methods). In our experiments, we show that this is the case. However, we stress that not regularizing critic might be controversial. A  suggestive straightforward example, present in the \cwtwenty{} sequence, is a situation when a task is repeated after a while, and the critic needs to be trained from scratch. %\maciejw{Maybe we should comment that there is no observed improvement in our case?}

We now present an in-depth analysis using EWC as an example. To this end, we performed a separate hyperparameter search for this setting for the regularization parameter $\lambda$ in \eqref{eq:generic_regularization}. Results, as presented in Figure \ref{fig:ewc_critic_ablation_appendix}, clearly indicate that the regularized cases struggle to achieve a decent result, in stark contrast to the non-regularized references (dashed lines) (we tested more values of $\lambda$, which are not included for better readability).% \maciejw{We tested more values of lambda and plot half of them for better readability.}

We consider critic regularization issues to be an important research direction.

% \piotrm{If available, it would be great to also other $\lambda$ for the non-regularized case. Possibly using dotted lines.}
% \maciejw{I'll try that, although I'd be a little bit worried about the clutter.}

% Here, we show empirical results showing this phenomenon, using the example of EWC. In case of this method (and all the considered regularization approaches), the decision to enable or disable critic regularization is easily implemented. We simply decide whether or not to sum over the critic parameters in the regularization loss function, see Equation \eqref{eq:generic_regularization}. %Such approach cannot be applied to methods from the replay family.


% In order to properly investigate the abilities of EWC with critic regularization, we performed a separate hyperparameter search for this setting, using the same range as for the EWC without critic regularization. The results are presented in Figure \ref{fig:ewc_critic_ablation_appendix}, with the EWC without regularization for comparison.
% The plot shows that none of the approaches with critic regularization performance come close to the base performance given by EWC without critic regularization. Using a critic which remembers how to learn on the task at hand should make training significantly faster. One would expect that regularizing the critic would show improvements when revisiting a given task, i.e. on tasks from 11 to 20. However, the results show no such phenomenon, implying that critic either failed to retain knowledge from the previous tasks (lack of stability) or is unable to use this knowledge well (lack of plasticity). Thus, we decide to drop critic regularization for all methods where it is possible.

% As we described in the main part of this work, we found that not regularizing the critic improves the result significantly.  Here, we show empirical results showing this phenomenon, using the example of EWC. In case of this method (and all the considered regularization approaches), the decision to enable or disable critic regularization is easily implemented. We simply decide whether or not to sum over the critic parameters in the regularization loss function, see Equation \eqref{eq:generic_regularization}. Such approach cannot be applied to methods from the replay family.


% In order to properly investigate the abilities of EWC with critic regularization, we performed a separate hyperparameter search for this setting, using the same range as for the EWC without critic regularization. The results are presented in Figure \ref{fig:ewc_critic_ablation_appendix}, with the EWC without regularization for comparison.
% The plot shows that none of the approaches with critic regularization performance come close to the base performance given by EWC without critic regularization. Using a critic which remembers how to learn on the task at hand should make training significantly faster. One would expect that regularizing the critic would show improvements when revisiting a given task, i.e. on tasks from 11 to 20. However, the results show no such phenomenon, implying that critic either failed to retain knowledge from the previous tasks (lack of stability) or is unable to use this knowledge well (lack of plasticity). Thus, we decide to drop critic regularization for all methods where it is possible.


% For example, the actor-critic framework commonly used in reinforcement learning offers additional trade-offs for continual learning methods, not seen in supervised learning. In this framework, the critic evaluates the decisions made by the actor, allowing him to learn which actions are preferable. Although the critic is required for the training, only the actor itself is needed to perform those actions well. As such for some methods we can decide to use the approach only on the actor and not on the critic. For example in, EWC we can manually zero out the Fisher weights for the critic, thus focusing only on actor regularization.

% We find that skipping the critic regularization leads to significantly better results, to the extent that some of the methods excel when they do not regularize the critic and fail catastrophically when they do. TODO: some exact numbers?

% However, for some approaches not regularizing the critic is simply not possible. For example, in the experience replay family of method we only remember the samples. There is not way of correctly using these samples if the critic does not remember the previous tasks.

% As such we chose not to regularize the critic where it's applicable in order to make the benchmark easier. Nonetheless, we argue that in the long term perspective regularizing the critic might be beneficial, as in real world applications it is often required to re-visit and retrain on a previously visited task.

\subsection{EWC Fisher matrix derivation}
\label{sec:ewc_fisher}
For the sake of completeness, we provide an analytical derivation of the Fisher matrix diagonal coefficients in the case of Gaussian distribution used by the SAC policy. In experiments presented in Section \ref{sec:critic_regularizaiton_appendix} we use these formulas also for the critic network assuming a normal distribution with constant $\sigma^2 = 1$.

\begin{fact}
    Let $\mu:\mathbb{R} \mapsto \mathbb{R}, \sigma:\mathbb{R} \mapsto \mathbb{R}$ parameterize a Gaussian distribution $\theta \mapsto \mathcal{N}\left(\mu(\theta), \sigma^2(\theta)\right)$. Then the diagonal of the Fisher information matrix $\mathcal{I}$ is
    \begin{equation} \label{eq:fisher_diagonal}
        \mathcal{I}_{kk} = \left(\frac{\partial \mu}{\partial \theta_k}\cdot\frac{1}{\sigma}\right)^{2}+
        2\left(\frac{\partial \sigma}{\partial \theta_k}\cdot\frac{1}{\sigma}\right)^{2}.
    \end{equation}
\end{fact}

Note that in SAC we use a factorized multivariate Gaussian distribution with mean vector $(\mu_1, \ldots, \mu_N)$ and standard deviations $(\sigma_1, \ldots, \sigma_N)$. It is straightforward to check that this case
\[
    \mathcal{I}_{kk} = \sum_{\ell=1}^N \left(\frac{\partial \mu_\ell}{\partial \theta_k}\cdot\frac{1}{\sigma_\ell}\right)^{2}+
    2\left(\frac{\partial \sigma_\ell}{\partial \theta_k}\cdot\frac{1}{\sigma_\ell}\right)^{2}.
\]

% EWC uses the Fisher information matrix to approximate the importance of each parameter in the network. Calculating the Fisher for classification problems, which are often considered in the supervised setting, is fairly trivial. However, calculating Fisher in the RL setting requires non-obvious assumptions and careful derivations, which we show here. \piotrm{I'd tune down, unless there is a clear non-trivial point. } \maciejw{I think it may be unclear that we assume that value function returns the mean of a Gaussian distribution, at least we discussed other possibilities before having feedback from Razvan. Other than that, I think all is clear.}


\input{fisher_derivation}


\subsection{VCL}% KL weight coefficient and prior for the first task}
\label{sec:vcl_problems_appendix}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/appendix/vcl_ablation.png}
    \caption{Average performance for VCL.}
    \label{fig:vcl_problems_appendix}
\end{figure}

We suggest introducing two changes to the original VCL setup \cite{DBLP:conf/iclr/NguyenLBT18}: treating $\lambda$ as hyperparameter and not using prior when training the first task. Our conclusion follows from the following three experimental evaluations:

% VCL was derived from the Bayesian perspective of maximizing likelihood along with incorporating strong priors. However, reinforcement learning is significantly different than usual MLE settings \maciejw{Is there a paper here which we can cite?}. Because of that and based on empirical evaluation we decided to introduce small changes to VCL. In this section we compare VCL as implemented in the original paper to VCL with our modified version adapted for the RL setting. In particular, we focus on two points which we changed: (1) performing a hyperparameter search for $\lambda$ instead of a fixed $\lambda$, and (2) not using the prior $\mathcal{N}(0, 1)$ when training on the first task.

% Thus, we consider three options in our experimental evaluation:
\begin{enumerate}
    \item Fixed $\lambda = 1/N$, where $N=10^6$ is the number of samples in each task.  The prior is applied during the first task.
    \item We tested the following hyperparameter values: $\lambda \in  \{ 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 10^0 \}$; selected value is $10^{-5}$.  The prior is applied during the first task.
          % $\lambda = 10^{-5}$ obtained via hyperparameter search from $\lambda \in  \{ 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 10^0 \}$\piotrm{change the order}.
    \item We tested the following hyperparameter values: $\lambda \in  \{ 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 10^0 \}$; selected value is $1$.  The prior is \emph{not} applied during the first task.
\end{enumerate}

The first setup is taken from \cite{DBLP:conf/iclr/NguyenLBT18}. As can be seen in Figure \ref{fig:vcl_problems_appendix} it underperformed, failing to keep good performance on previous tasks. Increasing $\lambda$ to $10^{-5}$ improves the results slightly. We observed that higher values of $\lambda$ fail due to strong regularization with respect to the initial prior. Abandoning this prior has led us to the most successful setup. Interestingly, the much higher value of $\lambda=1.0$ is optimal here. %\kucil{I would tone it down a little: ... gives good performance.}
% In Figure \ref{fig:vcl_problems_appendix} we show results on each of those settings. The approach most faithful to the original paper has the worst results, showing much worse performance even on the first task. The additional regularization makes it harder for the network to find right parameters. The second approach, where we perform hyperparameter search for the $\lambda$  coefficient to find $\lambda=10^{-5}$  shows slightly better results, although an interesting trade-off is present. After increasing the regularization coefficient ten-fold we are no longer able to learn the first task, since the model is more focused on keeping the weight distribution close to $\mathcal{N}(0, 1)$ than to learning new tasks. When we allow the model to skip the regularization during the first task, the model is able to use even larger coefficients with better results. Thus, we decide to incorporate these changes to VCL.


% VCL was derived from the Bayesian perspective of maximizing likelihood along with incorporating strong priors. However, reinforcement learning is significantly different than usual MLE settings \maciejw{Is there a paper here which we can cite?}. Because of that and based on empirical evaluation we decided to introduce small changes to VCL. In this section we compare VCL as implemented in the original paper to VCL with our modified version adapted for the RL setting. In particular, we focus on two points which we changed: (1) performing a hyperparameter search for $\lambda$ instead of a fixed $\lambda$, and (2) not using the prior $\mathcal{N}(0, 1)$ when training on the first task.

% Thus, we consider three options in our experimental evaluation:
% \begin{enumerate}
%     \item Fixed $\lambda = \frac{1}{N}$, where $N=10^6$ is the number of samples observed in each task. Additionally, KL regularization is applied during the first task.
%     \item $\lambda$ obtained through hyperparameter search, applying regularization during the first task.
%           % \item Fixed $\lambda$ obtained through hyperparameter search, applying regularization during the first task.
%     \item $\lambda$ obtained through hyperparameter search, not applying regularization during the first task.
% \end{enumerate}

% In Figure \ref{fig:vcl_problems_appendix} we show results on each of those settings. The approach most faithful to the original paper has the worst results, showing much worse performance even on the first task. The additional regularization makes it harder for the network to find right parameters. The second approach, where we perform hyperparameter search for the $\lambda$  coefficient to find $\lambda=10^{-5}$  shows slightly better results, although an interesting trade-off is present. After increasing the regularization coefficient ten-fold we are no longer able to learn the first task, since the model is more focused on keeping the weight distribution close to $\mathcal{N}(0, 1)$ than to learning new tasks. When we allow the model to skip the regularization during the first task, the model is able to use even larger coefficients with better results. Thus, we decide to incorporate these changes to VCL.



\subsection{Reservoir Sampling}
\label{sec:rsampling_appendix}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/appendix/reservoir_hps.png}
    \caption{The average performance of Reservoir Sampling. Note the $y$-axis scale change; $bs$ denotes the batch size.}
    \label{fig:reservoir_hps_appendix}
\end{figure}

We present more experiments for the Reservoir Sampling method. We vary the size of the replay $\in\{5\text{M}, 10\text{M}, 20\text{M}\}$. Recall that $20$M is enough to store the whole experience (which corresponds to the Perfect Memory experiments in the main section). For smaller sizes, we use reservoir sampling as described in Section \ref{sec:replay_methods_appendix}. We also test for different batch size values $\{64, 128, 256, 512\}$. We observe that higher values result in better performance, possibly due to better data balance in a single batch. This, however, comes at the cost of training speed.

Figure \ref{fig:reservoir_hps_appendix} shows results for different hyperparameter settings. Runs with the standard batch size $128$ used by the rest of the methods fail to exceed $0.05$ final average success obtained by Fine-tuning. Increasing the batch size improves the results significantly, and the two best runs using batch size $512$ achieve final average performance between $0.1$ and $0.15$. However, we note that even the best performing hyperparameters for Reservoir Sampling do not achieve as good results as the regularization and parameter isolation methods. We attribute this phenomenon to the critic regularization problem discussed in Section \ref{sec:critic_regularizaiton_appendix}.
% In the main section of the paper, we focused on a particular replay setting called perfect memory, where the agent is able to store all examples from the past. We also allowed the method to sample a larger number of samples from the buffer than in our standard setting (512 vs. 128), which improved results at cost of increased training speed. %Here, we show additional experiments without these assumptions. As explained in Section \ref{sec:replay_methods_appendix}, we use reservoir sampling to choose which samples should be in the buffer, instead of the standard FIFO approach of regular SAC.

\subsection{A-GEM not working}
\label{sec:agem_appendix}

Despite our best efforts, A-GEM has poor performance on our benchmark. In order to better investigate this case, we conduct additional analysis. In Figure~\ref{fig:agem_hparams} we show average performance on CW10 for various hyperparameter settings. We set the size of episodic task memory to 100k samples per task. We search for batch size (number of samples used to compute $\ell(\theta, \mathcal{B}_{new})$) in $\{ 128, 256, 512 \}$ and for the episodic batch size (number of samples used to compute $\ell(\theta, \mathcal{B}_{old})$) in $\{128, 256, 512, 1024 \}$, see \eqref{eq:agem_projection}. The results show that none of those settings perform significantly better than the others. Similar to Reservoir Sampling, we attribute those problems to the critic regularization discussed in Section \ref{sec:critic_regularizaiton_appendix}. Another conjecture is that due to the high variance of RL gradients (higher than in the supervfised learning setting), approximation \eqref{eq:agem_approx} is too brittle to work well.

% We also point to the fact that gradients in reinforcement learning are known to have high variance, which is not as problematic in supervised learning. This may in turn suggest that the approximation \eqref{eq:agem_approx} of the true constraint does not hold well enough in our setting. \maciejw{added some story. I'm not yet fully convinced about the gradient variance argument.}

\begin{figure}
    \begin{center}
        \includegraphics[width=\textwidth]{imgs/agem_hparams.png}
        \caption{\label{fig:agem_hparams} Average performance of A-GEM on CW10. Note the $y$-axis scale change. }
    \end{center}
\end{figure}

\subsection{PackNet extensive clipping} \label{sec:pack_net_appendix_problems}
Initially, PackNet was unstable, degenerating (NaNs and infinities) near the task boundaries. We amended this problem by applying global gradient norm clipping \num{2e-5}. We tune this value so that the learning does not explode and yet the performance is mostly preserved. PackNet instability requires further investigation: we conjecture that frequent changes of the set of optimized parameters might amplify the inherent instability of temporal-difference learning.


% Among the weights managed by PackNet, every task has an equal percentage reserved. All biases and normalization parameters (in LayerNorm) are not managed by PackNet; they remain frozen after learning of the first task. Also, last layer is not managed by PackNet. Every task has its own parameters there.

% Hyperparameter that we checked is number of retraining steps after each task (using only data from buffer). We searched among $\{50000, 100000, 200000\}$ and selected 100000.

% As a technical detail, we use global gradient norm clipping to the maximal value of $0.0001$. Without this clipping, learning explodes after several task changes.





==> 609bc59dc39be977132478d8 copy/cl_methods_short.tex <==
\section{Methods}\label{sec:cl_methods}
We now sketch $7$ CL methods evaluated on our benchmark. Some of them were developed for RL, while others were meant for the supervised learning context and required non-trivial adaptation.
%Most of them were developed in the SL context, and in some cases, non-trivial adaptation to the RL setting was required. 
We aimed to cover different families of methods; following \cite{de2019continual}, we consider three classes: regularization-based, parameter isolation and replay methods. An extended description and discussion of these methods are provided in Appendix \ref{sec:cl_methods_appendix}.

\textbf{Regularization-based Methods} This family builds on the observation that one can reduce forgetting by protecting parameters that are important for the previous tasks. The most basic approach often dubbed \textbf{L2}~\cite{DBLP:journals/corr/KirkpatrickPRVD16} simply adds a $L_2$ penalty, which regularizes the network not to stray away from the previously learned weights. In this approach, each parameter is equally important. \textbf{Elastic Weight Consolidation (EWC)}~\cite{DBLP:journals/corr/KirkpatrickPRVD16} uses the Fisher information matrix to approximate the importance of each weight.
%and propose a weighted $L_2$ penalty instead. 
\textbf{Memory-Aware Synapses (MAS)} \cite{DBLP:conf/eccv/AljundiBERT18} also utilizes a weighted penalty, but the importance is obtained by approximating the impact each parameter has on the output of the network. \textbf{Variational Continual Learning (VCL)}, follows a similar path but uses variational inference to minimize the Kullback-Leibler divergence between the current distribution of parameters (posterior) and the distribution for the previous tasks (prior).

\textbf{Parameter Isolation Methods} This family (also called modularity-based) forbids any changes to parameters that are important for the previous tasks. It may be considered as a ``hard'' equivalent of regularization-based methods. \textbf{PackNet}~\cite{DBLP:conf/cvpr/MallyaL18} ``packs'' multiple tasks into a single network by iteratively pruning, freezing, and retraining parts of the network at task change. PackNet is closely related to progressive neural networks \cite{DBLP:journals/corr/RusuRDSKKPH16},  developed in the RL context. 

\textbf{Replay Methods} Methods of this family keep some samples from the previous tasks and use them for training or as constraints to reduce forgetting. We use a \textbf{Perfect Memory} baseline, a modification of our setting which remembers all the samples from the past (i.e., without resetting the buffer at the task change). We also implemented \textbf{Averaged Gradient Episodic Memory (A-GEM)} \cite{DBLP:conf/iclr/ChaudhryRRE19}, which projects gradients from new samples as to not interfere with previous tasks. We find that A-GEM does not perform well on our benchmark. %We conjecture that stems from the fact that gradients in RL tend to be less informative.% and describe.% the problem in more detail in the appendix.


%Most CL methods were developed in the context of supervised learning. As a typical RL method is more conceptually complicated, new \piotrm{important} issues arise when adopting these CL methods. We now list most algorithmic points to be considered at the intersection of CL and RL. \piotrm{I think we'll put the below in the appendix, and here just a summary.}


%The high-level design of most (off-policy) RL algorithms (including SAC used in this work) consists of: ``actor'', ``critic'' and ``replay buffer.''
%\begin{itemize}
%    \item ``actor'' is a policy network. This the main object of interest -- only policy is used in evaluations. Compared to the standard RL setting, the policy network needs to be augmented with information about the task id. It can be injected as a one-hot vector or, in our case, as a separate network head. The actor is trained with an RL specific training loss. In L2, EWC, MAS, VCL this loss is supplemented by the specific loss associated with the respective method. In PackNet a short distillation phase is added, and some weights are not trainable, but otherwise, the actor training is unchanged. Reservoir sampling and A-GEM also do not require many changes (explained in the critic section).

%    \item ``critic'' represents the value function, numerical evaluation of states and actions. It might be considered as an auxiliary object helping in the actor training. In all but replay methods, we only need the critic corresponding to the current task. We found that \textit{not using} CL methods on the critic yields better results. We conjecture that as the previous tasks' value function is not needed,  it is better if the critic network maintains maximal plasticity. We found it beneficial to reset the critic's head; alternatively, the whole network can be reinitialized (but usually with worse performance) \maciejw{I would emphasize that we do not reset the critic in our standard setup.}\piotrm{why?} \maciejw{It kind of sounds like we do (since we claim it is better) and that might be confusing.} . In replay methods, we need to maintain critics related to the previous task. This necessitates changes in the critic architecture (we use multi-head akin to the actor) and using  CL methods to prevent forgetting. 
%    \item replay buffer - the SAC replay buffer is emptied whenever a new task begins. After that, we use a small warm-up period to fill the buffer. To this end, a uniform policy is used. (One could also use randomly initialized/new head). Resetting the replay buffer seems to have strong effects in toy one task experiments \piotrm{hint}. In replay methods, the old transitions are retained (tasks id needs to be stored in each sample).

%\end{itemize}

%\piotrm{List for discusssion - probably to be removed:}
%There are number of high-level challenges which the RL setting brings (or will eventually bring) to CL:
%\begin{itemize}
%    \item Exploration (high level) -- this might be a additional high level mechanism of forward transfer. That is the previous tasks might improve learning by providing more directed exploration.
%    \item Exploration (low level) -- it might be beneficial to increase exploration when task change (we do this little bit by putting random trajectories to the buffer)
%    \item Possibly use uncertainty estimates 
%    \item moving target - it not not completely clear, what to keep and what to forget (some suggest that forgetting is actually beneficial :))
%    \item Reward normalization - in the methods which use multi-task value function some reward normalization might be needed
%\item more hyperparamters - in the CL setting we do not want to change hyperparametrs when task change. In SL this is basically only LR in RL we have more, $\gamma$ and exploration temperature being most prominent
%    \item credit assignment - we have not intra-task credit assignment and inter task (seems stretched ;))
%    \item more complex setup - actor, critic (and buffer)
%\item Make some connections with off-line RL - possibly overstratched 
%    \item long-term planning - seems orthogonal to CL
%    \item brittleness 
%    \item sensitivity to hyperparmeters
% \item RL with uncertain rewards
%\end{itemize}

%SAC is a popular RL algorithm, known to be efficient in continuous domains. It follow the maximum entropy principle, which, in short, means that it favours slightly more stochastic policies. This is supposed to promote exploration and produce robust polices. SAC is an actor-critic algorithm, which means that it trains policy and the corresponding value function. SAC is an off-policy algorithm using replay buffer. 

% Relation to CL: \piotrm{list to discussion}
% \begin{itemize}
%     \item I do not particularly think that SAC is great for CL nor that it sucks ;)
%     \item Replay buffer is related to replay methods but I'd stay it is somewhat superficial \piotrm{In fact it is a good research direction to use replay as a source of expert data to behavioral cloning.}
%     \item SAC is considered to be quite stable (as for standards of continuous control RL)
%     \item It is not clear (?) what is better for CL, value based methods or policy methods. Policy. Testing value methods is possible, but not on this domain (DQN). There is no purely policy method with decent performance. 
% \end{itemize}

% \maciejw{highlight the less technical and more high-level problems of exploration, reward normalization, long-term planning etc. which do not occur in supervised learning. }\piotrm{Agreed. We need to find a more proper place for it.}

% \maciejw{Maybe we could consider moving subsection this to the experimental section? Most of these observation are empirical, i.e. we formed them after seeing the results. And Section 4 is already too long. 2021-01-30}
% While the majority of research in the field is done in the context of supervised learning, we argue that RL provides a more natural setting for CL, allowing for the sequential training protocol, non-stationary or changing environments, or meaningful task transitions. The RL setting also raises set of new conceptual and algorithmic challenges not present in the supervised setting.


% \piotrm{mw todo I think we should put a teaser of problems, possibly pointing to a method. However, we probably may laeve this until Section \ref{sec:cl_methods} is finished}

% \maciejw{Many algorithms did not work as it is (e.g. EWC required deriving Fisher with some non-obvious assumptions). I know that RL aspects are not really our focus, but maybe we could have a paragraph somewhere where we say that there were some issues and refer the reader to the appendix for details?}
% \maciejw{Continual learning methods perform much better when they do not regularize the critic, on the other hand it may be difficult to use them for retraining.}
% \maciejw{Experience replay methods, although they excel in supervised setting, do not perform very well in our benchmark. It maybe partly because they are forced to regularize the critic as well as the actor.}

==> 609bc59dc39be977132478d8 copy/cw20_results.tex <==
In Table \ref{tab:collected_resuls_appendix}, we recall for convenience the summary of our results for the experiments on the \cwtwenty{} sequence (additional backward transfer results are described in Section \ref{sec:forgetting_appendix}). We also recall that the methods were tuned with the objective of maximizing the final average performance. Our main findings are that most methods are efficient with mitigating forgetting but have an unsatisfying forward transfer. The best method, PackNet, has forward transfer close to Fine-tuning, which is a strong baseline for this metric. However, both fall below the reference value obtained from the analysis of the transfer matrix $\text{RT}=0.46$.

Table \ref{tab:collected_resuls_appendix} additionally highlights an important fact that CL metrics are interrelated. For instance, high forward transfer and low performance (a case for Fine-tuning and A-GEM) have to imply high forgetting.

\begin{table}[ht!]
    \begin{center}
        \tabcolsep=0.11cm
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}{lllll}
            \toprule
            method                  & performance                         & forgetting                  & f. transfer                         & b. transfer               \\
            \midrule
            \textbf{Fine-tuning}        & 0.05 {\tiny [0.05, 0.06]} & 0.73 {\tiny [0.72, 0.75]}   & \textbf{0.20 {\tiny [0.17, 0.23]}} & 0.00 {\tiny[0.00, 0.00]} \\
            \textbf{L2}          & 0.43 {\tiny [0.39, 0.47]} & 0.02 {\tiny [0.00, 0.03]}   & -0.71 {\tiny [-0.87, -0.57]}      & 0.02 {\tiny[0.02, 0.03]} \\
            \textbf{EWC}         & 0.60 {\tiny [0.57, 0.64]} & 0.02 {\tiny [-0.00, 0.05]}  & -0.17 {\tiny [-0.24, -0.11]}       & 0.04 {\tiny[0.03, 0.04]} \\
            \textbf{MAS}         & 0.51 {\tiny [0.49, 0.53]} & 0.00 {\tiny [-0.01, 0.02]}  & -0.52 {\tiny [-0.59, -0.47]}      & 0.04 {\tiny[0.04, 0.05]} \\
            \textbf{VCL}         & 0.48 {\tiny [0.46, 0.50]} & 0.01 {\tiny [-0.01, 0.02]}  & -0.49 {\tiny [-0.57, -0.42]}       & 0.04 {\tiny[0.03, 0.04]} \\
            \textbf{PackNet}     & \textbf{0.80 {\tiny [0.79, 0.82]}} & 0.00 {\tiny [-0.01, 0.01]} & \textbf{0.19 {\tiny [0.15, 0.23]}} & 0.03 {\tiny[0.03, 0.04]} \\
            \textbf{Perfect Memory}   & 0.12 {\tiny [0.09, 0.15]} & 0.07 {\tiny [0.05, 0.10]}   & -1.34 {\tiny [-1.42, -1.27]}       & 0.01 {\tiny[0.01, 0.01]} \\
            \textbf{A-GEM}        & 0.07 {\tiny [0.06, 0.08]} & 0.71 {\tiny [0.70, 0.73]}   & 0.13 {\tiny [0.10, 0.16]}          & 0.00 {\tiny[0.00, 0.00]} \\
            \midrule
            \textbf{MT}         & 0.51 {\tiny [0.48, 0.53]} & ---                 & ---                                 & ---                       \\
            \textbf{MT (PopArt)}  & 0.65 {\tiny [0.63, 0.67]} & ---                 & ---                                 & ---                       \\
            \midrule
            \textbf{RT}             & ---                                 & ---                         & \textbf{0.46}                       & ---                       \\
            \bottomrule
        \end{tabular}
        \caption{Results on \cwtwenty{}, for CL methods and multi-task training.}
        \label{tab:collected_resuls_appendix}
    \end{center}
\end{table}

We recall that CW10 and CW20 sequences are defined in Section \ref{sec:sequences_appendix}. In the next sections, we discuss the results in more detail. We also provide the following visualizations:
\begin{itemize}
    \item Figure \ref{sec:average_success_big} - performance curves averaged over tasks.
    \item Figure \ref{fig:current_task_big} - performance curves for the active task.
    \item Figure \ref{sec:task_success_big} - performance curves for all tasks. Useful for qualitative studies of transfer and forgetting.
    \item Figure \ref{fig:foraward_transfer_per_task} - visualization of forward transfer for each task.
    \item Figure \ref{fig:forgetting_big_plot} - forgetting curves averaged over tasks.
\end{itemize}

% \piotrm{Possibly make list of figures.}

% \kucil{pull with stick, place shelf, hammer, unplug peg have the "richest" reward structure (reach, grasp, place). from hammer (and from push back) transfer is positive (transfer matrix)}

\subsection{Forgetting and backward transfer} \label{sec:forgetting_appendix}
%Recall Table \ref{tab:collected_resuls_appendix},  in 
Table \ref{tab:forgetting_table} expands upon Table \ref{tab:collected_resuls_appendix}   by presenting more detailed forgetting results, see also Figure \ref{fig:forgetting_big_plot} and Figure \ref{sec:task_success_big}. The latter is convenient to observe the evaluation dynamics of each task.

Fine-tuning and AGEM exhibit rapid catastrophic forgetting after task switch (see Figure \ref{sec:task_success_big}). It is expected for the former, but quite surprising for the latter. We conjecture possible reasons in Section \ref{sec:agem_appendix}. Some mild forgetting can also be observed for Perfect Memory (it is not directly observed in the metric due to the poor training but can be visible on the graphs). The rest of the methods are quite efficient in mitigating forgetting. This also includes the very basic L2 method (which is at the cost of poor transfer, however).


In our experiment, we do not observe backward transfer, see Table \ref{tab:collected_resuls_appendix}. The values were calculated according to $B := \frac{1}{N}\sum_{i=1}^N B_i$, where
\[
    B_i := \max\left\{0,  p_i(T) - p_i(i\cdot \Delta)\right\},
\]
see Section \ref{sec:metrics} for notation. Note that some small values are possible due to stochastic evaluations.

\begin{table}[h]
    \centering
    \scriptsize
    \rotatebox{90}{
    \begin{tabular}{lllllllll}
        \toprule
        task & Fine-tuning       & L2                   & EWC                  & MAS                  & VCL                  & PackNet              & Perfect Memory      & A-GEM             \\
        \midrule
        0    & 0.86 [0.82, 0.90] & 0.07 [-0.04, 0.19]   & 0.38 [0.23, 0.53]    & -0.02 [-0.07, 0.04]  & -0.05 [-0.10, 0.01]  & -0.01 [-0.09, 0.06]  & 0.56 [0.48, 0.64]   & 0.86 [0.82, 0.91] \\
        1    & 0.72 [0.67, 0.77] & 0.08 [0.02, 0.14]    & 0.04 [-0.04, 0.13]   & 0.01 [-0.07, 0.08]   & 0.04 [-0.02, 0.09]   & -0.03 [-0.07, 0.00]  & 0.29 [0.19, 0.40]   & 0.78 [0.72, 0.83] \\
        2    & 0.91 [0.88, 0.95] & 0.09 [0.01, 0.18]    & 0.01 [-0.05, 0.08]   & 0.01 [-0.07, 0.09]   & 0.01 [-0.05, 0.07]   & -0.03 [-0.06, -0.01] & 0.07 [0.03, 0.12]   & 0.92 [0.88, 0.96] \\
        3    & 0.99 [0.98, 0.99] & -0.00 [-0.02, 0.02]  & 0.04 [0.01, 0.07]    & 0.00 [-0.07, 0.08]   & -0.04 [-0.08, -0.00] & -0.01 [-0.01, -0.00] & 0.04 [0.00, 0.12]   & 0.98 [0.96, 0.99] \\
        4    & 0.67 [0.55, 0.77] & -0.01 [-0.03, 0.00]  & -0.03 [-0.08, 0.02]  & -0.10 [-0.17, -0.05] & -0.01 [-0.03, 0.01]  & -0.03 [-0.09, 0.02]  & 0.00 [0.00, 0.00]   & 0.76 [0.67, 0.84] \\
        5    & 0.96 [0.95, 0.97] & -0.01 [-0.03, 0.00]  & 0.01 [-0.06, 0.11]   & -0.01 [-0.10, 0.07]  & 0.13 [0.01, 0.25]    & -0.02 [-0.03, 0.00]  & 0.04 [-0.01, 0.08]  & 0.97 [0.95, 0.99] \\
        6    & 0.83 [0.80, 0.86] & 0.02 [-0.02, 0.06]   & 0.02 [-0.02, 0.06]   & 0.04 [0.00, 0.08]    & -0.00 [-0.05, 0.05]  & 0.04 [-0.00, 0.09]   & 0.00 [0.00, 0.00]   & 0.78 [0.75, 0.81] \\
        7    & 0.54 [0.44, 0.64] & 0.01 [-0.02, 0.05]   & 0.01 [-0.04, 0.06]   & 0.01 [-0.02, 0.04]   & -0.02 [-0.06, 0.02]  & 0.06 [-0.00, 0.13]   & 0.00 [0.00, 0.00]   & 0.66 [0.49, 0.80] \\
        8    & 0.87 [0.83, 0.90] & -0.01 [-0.03, 0.02]  & 0.02 [-0.07, 0.12]   & 0.07 [-0.01, 0.17]   & -0.06 [-0.12, 0.01]  & -0.00 [-0.02, 0.01]  & 0.01 [-0.07, 0.08]  & 0.89 [0.84, 0.94] \\
        9    & 0.97 [0.96, 0.98] & 0.01 [-0.01, 0.04]   & -0.00 [-0.01, 0.00]  & 0.03 [-0.04, 0.11]   & 0.11 [0.03, 0.20]    & 0.00 [-0.00, 0.01]   & 0.01 [-0.02, 0.04]  & 0.93 [0.88, 0.98] \\
        10   & 0.67 [0.54, 0.80] & 0.05 [0.00, 0.12]    & -0.08 [-0.12, -0.04] & -0.01 [-0.03, 0.01]  & 0.05 [0.00, 0.12]    & -0.02 [-0.06, 0.03]  & 0.00 [0.00, 0.00]   & 0.66 [0.47, 0.82] \\
        11   & 0.54 [0.49, 0.59] & 0.04 [0.01, 0.07]    & -0.01 [-0.06, 0.04]  & -0.01 [-0.05, 0.03]  & -0.00 [-0.02, 0.02]  & 0.08 [0.01, 0.15]    & 0.00 [0.00, 0.00]   & 0.42 [0.32, 0.50] \\
        12   & 0.83 [0.78, 0.87] & 0.02 [-0.02, 0.06]   & 0.00 [-0.05, 0.07]   & -0.01 [-0.04, 0.02]  & -0.01 [-0.05, 0.03]  & 0.00 [-0.03, 0.04]   & 0.00 [0.00, 0.01]   & 0.70 [0.60, 0.80] \\
        13   & 0.98 [0.97, 0.99] & 0.01 [0.00, 0.02]    & -0.02 [-0.06, 0.01]  & -0.00 [-0.03, 0.02]  & -0.00 [-0.04, 0.04]  & -0.00 [-0.01, 0.01]  & 0.00 [0.00, 0.00]   & 0.95 [0.89, 0.99] \\
        14   & 0.36 [0.23, 0.49] & 0.00 [0.00, 0.00]    & -0.02 [-0.04, 0.00]  & -0.01 [-0.02, 0.00]  & 0.00 [-0.00, 0.00]   & -0.02 [-0.05, 0.01]  & 0.00 [0.00, 0.00]   & 0.36 [0.18, 0.55] \\
        15   & 0.95 [0.94, 0.97] & -0.02 [-0.06, 0.02]  & 0.09 [0.02, 0.18]    & 0.08 [-0.00, 0.18]   & 0.08 [-0.01, 0.18]   & -0.00 [-0.02, 0.02]  & -0.00 [-0.04, 0.03] & 0.97 [0.95, 0.98] \\
        16   & 0.63 [0.57, 0.69] & 0.00 [-0.03, 0.03]   & -0.01 [-0.04, 0.03]  & -0.01 [-0.05, 0.03]  & -0.02 [-0.05, 0.00]  & -0.03 [-0.06, 0.01]  & 0.00 [0.00, 0.00]   & 0.55 [0.49, 0.61] \\
        17   & 0.46 [0.38, 0.55] & -0.02 [-0.05, -0.00] & 0.00 [-0.02, 0.03]   & 0.00 [-0.01, 0.01]   & -0.01 [-0.03, 0.00]  & -0.05 [-0.09, -0.00] & 0.00 [0.00, 0.00]   & 0.43 [0.30, 0.56] \\
        18   & 0.93 [0.90, 0.96] & 0.02 [-0.03, 0.08]   & -0.03 [-0.06, -0.01] & -0.01 [-0.04, 0.02]  & -0.03 [-0.07, 0.01]  & 0.01 [-0.01, 0.04]   & -0.04 [-0.09, 0.01] & 0.88 [0.81, 0.94] \\
        19   & 0.00 [0.00, 0.00] & 0.00 [0.00, 0.00]    & 0.00 [0.00, 0.00]    & 0.00 [0.00, 0.00]    & 0.00 [0.00, 0.00]    & 0.00 [0.00, 0.00]    & 0.00 [0.00, 0.00]   & 0.00 [0.00, 0.00] \\
        \midrule
        mean & 0.73 [0.72, 0.75] & 0.02 [0.00, 0.03]    & 0.02 [-0.00, 0.05]   & 0.00 [-0.01, 0.02]   & 0.01 [-0.01, 0.02]   & -0.00 [-0.01, 0.01]  & 0.05 [0.04, 0.06]   & 0.72 [0.71, 0.74] \\
        \bottomrule
    \end{tabular}}
    \caption{Forgetting for each method (columns) and tasks (rows). } \label{tab:forgetting_table}
\end{table}


\subsection{Forward transfer} \label{sec:forward_transfer_appendix}
Table \ref{tab:transfer_table} and Figure \ref{fig:transfer_heatmap} supplement Table \ref{tab:collected_resuls_appendix} with detailed results on forward transfer on \cwtwenty{}. Corresponding training curves can be find in Figure \ref{fig:foraward_transfer_per_task} and Figure \ref{fig:current_task_big}.

Fine-tuning is a strong baseline, with PackNet and AGEM taking close second and third place (although the latter method has a low overall performance). Unfortunately, all the other methods suffer from the negative forward transfer, which in all cases, except possibly from EWC, is quite significant. To make the picture grimmer, transfer on the second part of \cwtwenty{} is worse, even though the task has been learned (and not forgotten) on the first part, see Table \ref{tab:negative_transfer_delta}.

% \kucil{Average transfer over methods, for each task: [0.08, -0.26, 0.07, 0.21, -0.26, -0.43, -1.11, 0.0, -0.15, -0.26, -0.54, -0.57, -0.45, 0.02, -0.38, -0.46, -1.74, -0.14, -0.25, -0.26]}

\begin{figure}
    \begin{center}
        \includegraphics[width=\textwidth]{imgs/transfer_heatmap_cw20.png}
        \caption{Forward transfer heatmap for CW20. The shaded cells indicate that $0$ belongs to the corresponding $90\%$ confidence interval. }\label{fig:transfer_heatmap}
    \end{center}
\end{figure}


\begin{table}[h]
    \centering
    \scriptsize 
    \rotatebox{90}{
    \begin{tabular}{llllllllll}
        \toprule
        Method & Fine-tuning                 & L2                           & EWC                          & MAS                          & VCL                          & PackNet                     & Perfect Memory               & A-GEM                     & mean  \\
        Task   &                             &                              &                              &                              &                              &                             &                              &                           &       \\
        \midrule
        0      & 0.13 [0.05, 0.20]           & 0.14 [0.07, 0.21]            & 0.13 [0.05, 0.20]            & 0.13 [0.05, 0.20]            & 0.02 [-0.09, 0.12]           & -0.49 [-0.65, -0.34]        & 0.43 [0.31, 0.54]            & 0.13 [0.04, 0.22]         & 0.08  \\
        1      & 0.06 [-0.09, 0.18]          & -0.39 [-0.53, -0.25]         & -0.10 [-0.19, -0.02]         & -0.63 [-0.72, -0.54]         & -0.51 [-0.60, -0.40]         & -0.08 [-0.19, 0.03]         & -0.68 [-0.83, -0.52]         & 0.21 [0.14, 0.28]         & -0.26 \\
        2      & 0.39 [0.23, 0.52]           & -0.09 [-0.40, 0.19]          & 0.35 [0.20, 0.49]            & 0.04 [-0.20, 0.24]           & -0.09 [-0.36, 0.14]          & 0.33 [0.09, 0.51]           & -0.82 [-1.18, -0.51]         & 0.48 [0.37, 0.58]         & 0.07  \\
        3      & 0.76 [0.73, 0.79]           & -0.26 [-0.53, -0.01]         & 0.66 [0.51, 0.76]            & -0.09 [-0.31, 0.13]          & -0.33 [-0.58, -0.12]         & 0.80 [0.76, 0.83]           & -0.71 [-0.91, -0.53]         & 0.81 [0.78, 0.83]         & 0.21  \\
        4      & 0.08 [-0.05, 0.20]          & -0.45 [-0.52, -0.38]         & -0.36 [-0.45, -0.26]         & -0.35 [-0.45, -0.25]         & -0.48 [-0.54, -0.42]         & -0.21 [-0.33, -0.09]        & -0.49 [-0.55, -0.43]         & 0.18 [0.05, 0.29]         & -0.26 \\
        5      & 0.55 [0.50, 0.59]           & -1.84 [-2.39, -1.29]         & 0.14 [0.04, 0.24]            & -0.44 [-0.59, -0.29]         & -0.38 [-0.58, -0.20]         & 0.05 [-0.22, 0.29]          & -1.96 [-2.41, -1.49]         & 0.45 [0.30, 0.57]         & -0.43 \\
        6      & -0.11 [-0.24, 0.00]         & -1.69 [-1.94, -1.44]         & -0.81 [-0.98, -0.62]         & -1.38 [-1.60, -1.17]         & -1.81 [-1.97, -1.65]         & 0.12 [0.04, 0.20]           & -2.92 [-3.05, -2.80]         & -0.27 [-0.38, -0.17]      & -1.11 \\
        7      & 0.13 [0.04, 0.22]           & -0.20 [-0.26, -0.15]         & -0.10 [-0.19, -0.01]         & -0.18 [-0.24, -0.12]         & -0.10 [-0.17, -0.03]         & 0.44 [0.34, 0.53]           & -0.24 [-0.29, -0.19]         & 0.28 [0.14, 0.42]         & 0.00  \\
        8      & 0.44 [0.38, 0.50]           & -0.91 [-1.45, -0.38]         & 0.35 [0.21, 0.47]            & -0.18 [-0.56, 0.14]          & 0.12 [-0.17, 0.35]           & 0.45 [0.29, 0.58]           & -1.86 [-2.20, -1.53]         & 0.41 [0.27, 0.54]         & -0.15 \\
        9      & 0.77 [0.70, 0.81]           & -0.68 [-1.20, -0.25]         & -0.11 [-0.64, 0.32]          & -0.51 [-1.05, -0.05]         & -0.66 [-1.21, -0.17]         & 0.80 [0.72, 0.86]           & -2.44 [-3.05, -1.95]         & 0.79 [0.73, 0.84]         & -0.26 \\
        10     & -0.30 [-0.60, -0.01]        & -0.49 [-0.82, -0.15]         & -0.66 [-0.96, -0.36]         & -0.41 [-0.74, -0.10]         & -0.07 [-0.35, 0.19]          & -0.41 [-0.74, -0.10]        & -1.73 [-1.85, -1.63]         & -0.23 [-0.67, 0.16]       & -0.54 \\
        11     & -0.21 [-0.30, -0.12]        & -0.77 [-0.90, -0.65]         & -0.57 [-0.70, -0.45]         & -0.71 [-0.81, -0.61]         & -0.91 [-1.01, -0.80]         & 0.08 [-0.02, 0.17]          & -1.07 [-1.15, -1.00]         & -0.43 [-0.61, -0.25]      & -0.57 \\
        12     & 0.04 [-0.14, 0.20]          & -0.74 [-1.09, -0.43]         & -0.36 [-0.68, -0.08]         & -0.67 [-1.00, -0.38]         & -0.38 [-0.66, -0.13]         & 0.42 [0.32, 0.50]           & -1.76 [-2.11, -1.48]         & -0.19 [-0.47, 0.06]       & -0.45 \\
        13     & 0.53 [0.44, 0.60]           & -0.59 [-0.79, -0.41]         & 0.39 [0.25, 0.51]            & -0.33 [-0.55, -0.13]         & -0.44 [-0.67, -0.22]         & 0.82 [0.79, 0.85]           & -0.78 [-0.96, -0.64]         & 0.56 [0.44, 0.67]         & 0.02  \\
        14     & -0.19 [-0.31, -0.05]        & -0.49 [-0.55, -0.43]         & -0.47 [-0.53, -0.41]         & -0.45 [-0.53, -0.37]         & -0.49 [-0.55, -0.43]         & -0.24 [-0.35, -0.13]        & -0.49 [-0.55, -0.43]         & -0.25 [-0.41, -0.09]      & -0.38 \\
        15     & 0.48 [0.41, 0.56]           & -1.52 [-1.99, -1.08]         & 0.03 [-0.13, 0.19]           & -1.05 [-1.40, -0.73]         & -0.20 [-0.41, -0.01]         & 0.17 [-0.00, 0.34]          & -1.94 [-2.44, -1.44]         & 0.36 [0.24, 0.48]         & -0.46 \\
        16     & -0.79 [-0.96, -0.63]        & -2.44 [-2.64, -2.26]         & -1.83 [-2.07, -1.59]         & -2.07 [-2.28, -1.85]         & -2.50 [-2.68, -2.33]         & -0.34 [-0.48, -0.19]        & -2.92 [-3.05, -2.80]         & -1.05 [-1.23, -0.86]      & -1.74 \\
        17     & 0.02 [-0.07, 0.11]          & -0.23 [-0.28, -0.18]         & -0.20 [-0.26, -0.13]         & -0.22 [-0.28, -0.17]         & -0.22 [-0.28, -0.17]         & -0.03 [-0.12, 0.06]         & -0.24 [-0.29, -0.19]         & -0.03 [-0.13, 0.09]       & -0.14 \\
        18     & 0.52 [0.45, 0.58]           & -0.74 [-1.23, -0.30]         & -0.06 [-0.46, 0.28]          & -0.67 [-1.19, -0.17]         & 0.26 [-0.04, 0.49]           & 0.44 [0.28, 0.58]           & -2.24 [-2.57, -1.86]         & 0.52 [0.46, 0.58]         & -0.25 \\
        19     & 0.73 [0.66, 0.78]           & -0.59 [-1.08, -0.18]         & -0.16 [-0.71, 0.29]          & -0.26 [-0.77, 0.13]          & -0.45 [-1.02, 0.03]          & 0.46 [0.12, 0.70]           & -2.49 [-3.11, -1.98]         & 0.68 [0.58, 0.75]         & -0.26 \\
        \midrule
        mean   & {0.20 {\tiny [0.17, 0.23]}} & -0.75 {\tiny [-0.87, -0.65]} & -0.19 {\tiny [-0.25, -0.14]} & -0.52 {\tiny [-0.58, -0.48]} & -0.48 {\tiny [-0.56, -0.42]} & {0.18 {\tiny [0.14, 0.21]}} & -1.37 {\tiny [-1.46, -1.30]} & 0.17 {\tiny [0.13, 0.20]} & ---   \\
        \bottomrule
    \end{tabular}}
    \caption{Forward transfers on \cwtwenty{} (rows) for each method (columns).} \label{tab:transfer_table}
    %\label{tab:my_label}
\end{table}

\begin{table}[h]
    \centering\small
    \begin{tabular}{lrrrrrrrrrr}
        \toprule
        Task           & $\Delta_0$ & $\Delta_1$ & $\Delta_2$ & $\Delta_3$ & $\Delta_4$ & $\Delta_5$ & $\Delta_6$ & $\Delta_7$ & $\Delta_8$ & $\Delta_9$ \\
        Method         &            &            &            &            &            &            &            &            &            &            \\
        \midrule
        Fine-tuning    & -0.42      & -0.27      & -0.34      & -0.24      & -0.26      & -0.06      & -0.68      & -0.11      & 0.08       & -0.04      \\
        L2             & -0.63      & -0.39      & -0.66      & -0.33      & -0.03      & 0.32       & -0.76      & -0.02      & 0.17       & 0.10       \\
        EWC            & -0.79      & -0.47      & -0.71      & -0.27      & -0.11      & -0.11      & -1.02      & -0.09      & -0.41      & -0.05      \\
        MAS            & -0.54      & -0.08      & -0.71      & -0.24      & -0.10      & -0.61      & -0.68      & -0.04      & -0.49      & 0.25       \\
        VCL            & -0.08      & -0.40      & -0.29      & -0.11      & -0.01      & 0.18       & -0.69      & -0.13      & 0.13       & 0.20       \\
        PackNet        & 0.09       & 0.16       & 0.08       & 0.02       & -0.03      & 0.12       & -0.46      & -0.47      & -0.01      & -0.34      \\
        Perfect Memory & -2.16      & -0.39      & -0.94      & -0.07      & 0.00       & 0.02       & 0.00       & 0.00       & -0.38      & -0.05      \\
        A-GEM          & -0.36      & -0.63      & -0.67      & -0.25      & -0.43      & -0.09      & -0.77      & -0.32      & 0.11       & -0.11      \\
        \bottomrule
    \end{tabular}
    \caption{Difference in transfer when revisiting tasks. $\Delta_i = \text{FT}_{i+10} - \text{FT}_i$; recall that $i$ and $i+10$ are the same tasks in \cwtwenty{}.} \label{tab:negative_transfer_delta}
    %\label{tab:my_label}
\end{table}

\subsection{Results for CW10}
In Table~\ref{tab:cw10} we present results for the CW10 sequence ($10$ task version of the benchmark, without repeating the tasks). One can see that results are mostly consistent with \cwtwenty{} (see Table \ref{tab:collected_resuls_appendix}), and thus CW10 can be used for faster experimenting. More detailed transfer results can be found in Table \ref{tab:transfer_table}.

\begin{table}[th]
    \begin{center}
        \tabcolsep=0.11cm
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}{llll}
\toprule
 method   & performance       & forgetting           & f. transfer   \\
\midrule
 \textbf{Fine-tuning}        & 0.10 {\tiny [0.10, 0.11]} & 0.74 {\tiny [0.72, 0.75]}    & \textbf{0.32 {\tiny [0.28, 0.35]}}     \\
 \textbf{L2}          & 0.48 {\tiny [0.43, 0.53]} & 0.02 {\tiny [-0.00, 0.04]}   & -0.57 {\tiny [-0.77, -0.39]}  \\
 \textbf{EWC}         & 0.66 {\tiny [0.62, 0.69]} & 0.03 {\tiny [0.01, 0.06]}    & 0.05 {\tiny [-0.02, 0.12]}    \\
 \textbf{MAS}         & 0.59 {\tiny [0.56, 0.61]} & -0.02 {\tiny [-0.03, -0.00]} & -0.35 {\tiny [-0.42, -0.28]}  \\
 \textbf{VCL}         & 0.53 {\tiny [0.49, 0.58]} & -0.02 {\tiny [-0.03, -0.00]} & -0.44 {\tiny [-0.57, -0.32]}  \\
 \textbf{PackNet}     & \textbf{0.83 {\tiny [0.81, 0.85]}} & -0.00 {\tiny [-0.01, 0.01]}  & 0.21 {\tiny [0.16, 0.25]}     \\
 \textbf{Perfect Memory}   & 0.29 {\tiny [0.26, 0.31]} & 0.03 {\tiny [0.02, 0.05]}    & -1.11 {\tiny [-1.20, -1.04]}  \\
 \textbf{A-GEM}        & 0.13 {\tiny [0.12, 0.14]} & 0.73 {\tiny [0.72, 0.75]}    & \textbf{0.29 {\tiny [0.27, 0.32]}}     \\
 \midrule
 \textbf{MT}         & 0.51 {\tiny [0.48, 0.53]} & ---                  & ---                   \\
 \textbf{MT (PopArt)}  & 0.65 {\tiny [0.63, 0.67]} & ---                  & ---                   \\
            \bottomrule
        \end{tabular}
        \caption{Results on CW10, for CL methods and multi-task training.}
        \label{tab:cw10}
    \end{center}
\end{table}


% % In practice because we have only a finite amount of samples we approximate the integral with a sum. Please note that since success rate $p \in [0, 1]$ is bounded, then the maximal forward transfer achievable is $1$. However, this transfer is not bounded from below.

% \piotrm{todo: put also results of the baseline training, i.e. $\text{AUC}_i^b$ from definition \eqref{eq:noramlized_forward_transfer}}

% Average forward transfer presented in Table \ref{tab:long_forward_transfer_table} highlight that most of the methods are able to mitigate forgetting at the cost of decreasing forward transfer. The only exception here is PackNet, which maintains good forward transfer throughout the first ten tasks. However, when the second ten tasks start, PackNet's performance degrades as well, potentially due to lack of capacity.

% \begin{figure*}[h!]
%     \vskip 0.2in
%     \begin{center}
%         \centerline{\includegraphics[width=\textwidth]{imgs/all_new.png}}
%         \caption{Transfer heatmap: all} \label{fig:transfer_all}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}

% \input{long_transfer_tables.tex}

% \begin{figure*}[ht!]
%     \vskip 0.2in
%     \begin{center}
%         \centerline{\includegraphics[width=0.6\textwidth]{imgs/first_ten_new.png}}
%         \caption{Transfer heatmap: first 10} \label{fig:transfer_first_10}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}

% \begin{figure*}[ht!]
%     \vskip 0.2in
%     \begin{center}
%         \centerline{\includegraphics[width=.6\textwidth]{imgs/second_ten_new.png}}
%         \caption{Transfer heatmap: second 10} \label{fig:transfer_second_10}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}



% \piotrm{Possibly put transfer graphs for all methods}
% We illustrate forward transfer of a vanilla method and PackNet in Figures \ref{fig:vanilla_ft} and \ref{fig:packnet_ft} respectively.

% \begin{figure*}[ht!]
%     \vskip 0.2in
%     \begin{center}
%         \centerline{\includegraphics[width=\textwidth]{imgs/plot_forward_transfer_vanilla.png}}
%         \caption{\textbf{Forward Transfer on 20 tasks for Vanilla Method}.}
%         \label{fig:vanilla_ft}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}
% \clearpage
% \newpage


==> 609bc59dc39be977132478d8 copy/experiments.tex <==
Now we present empirical results; these are evaluations of a set of $7$ representative CL methods (as described in Section \ref{sec:cl_methods}) on our Continual World benchmark.  We focus on \textit{forgetting and transfers} while keeping fixed constraints on computation, memory, number of samples, and neural network architecture. Our main empirical contributions are experiments on the long CW20 sequence and following high-level conclusions. 
%We believe they are of importance for the field. 
For a summary see Table \ref{tab:collected_resuls}, Figure \ref{fig:training_graph} and for an extensive discussion, we refer to Appendix \ref{sec:cwtwenty_graph_and_analysis_appendix} (including results for the shorter sequence, CW10). In Appendix \ref{sec:ablations_appendix} we provide various ablations and detailed analysis of sensitivity to the CL-specific hyperparameters.

% \begin{table}[t]
\begin{wraptable}{r}{0.65\linewidth}
    \vskip -0.2in
    \begin{center}
        \small
        \tabcolsep=0.11cm
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llll}
\toprule
 method   & performance       & forgetting          & f. transfer   \\
\midrule
 \textbf{Fine-tuning}        & 0.05 {\tiny [0.05, 0.06]} & 0.73 {\tiny [0.72, 0.75]}   & \textbf{0.20 {\tiny [0.17, 0.23]}}     \\
 \textbf{L2}          & 0.43 {\tiny [0.39, 0.47]} & 0.02 {\tiny [0.00, 0.03]}   & -0.71 {\tiny [-0.87, -0.57]}  \\
 \textbf{EWC}         & 0.60 {\tiny [0.57, 0.64]} & 0.02 {\tiny [-0.00, 0.05]}  & -0.17 {\tiny [-0.24, -0.11]}  \\
 \textbf{MAS}         & 0.51 {\tiny [0.49, 0.53]} & 0.00 {\tiny [-0.01, 0.02]}  & -0.52 {\tiny [-0.59, -0.47]}  \\
 \textbf{VCL}         & 0.48 {\tiny [0.46, 0.50]} & 0.01 {\tiny [-0.01, 0.02]}  & -0.49 {\tiny [-0.57, -0.42]}  \\
 \textbf{PackNet}     & \textbf{0.80 {\tiny [0.79, 0.82]}} & 0.00 {\tiny [-0.01, 0.01]} & \textbf{0.19 {\tiny [0.15, 0.23]}}     \\
 \textbf{Perfect Memory}   & 0.12 {\tiny [0.09, 0.15]} & 0.07 {\tiny [0.05, 0.10]}   & -1.34 {\tiny [-1.42, -1.27]}  \\
 \textbf{A-GEM}        & 0.07 {\tiny [0.06, 0.08]} & 0.71 {\tiny [0.70, 0.73]}   & 0.13 {\tiny [0.10, 0.16]}     \\
\midrule
 \textbf{MT}         & 0.51 {\tiny [0.48, 0.53]} & ---                 & ---                   \\
 \textbf{MT (PopArt)}  & 0.65 {\tiny [0.63, 0.67]} & ---                 & ---                   \\
            \midrule
            \textbf{RT}          & ---                                & ---                         & \textbf{0.46}                             \\
            \bottomrule
        \end{tabular}
        \caption{\small Results on \cwtwenty{}, for CL methods and multi-task training.  Metrics are defined in Section \ref{sec:metrics}, RT is eq. \eqref{eq:forward_transfer_upperbound}. We used $20$ seeds and provide 90\% confidence intervals. } %\michal{I wonder if these refs to equations are really helpful, especially since the distance in text is big... Maybe instead write "performance, forgetting, tranfsfer as defined in Section X?} 
        \label{tab:collected_resuls}
    \end{center}
    \vskip -0.3in
\end{wraptable}
% \end{table}

\textbf{Performance} The performance (success rate) averaged over tasks (eq. \eqref{eq:performance}) is a typical metric for the CL setting. PackNet seems to outperform other methods, approaching $0.8$ from the maximum of $1.0$, outperforming multi-task solutions which might struggle with different reward scales, a problem elegantly avoided in the CL framing. Other methods perform considerably worse. A-GEM and Perfect Memory struggle. We further discuss possible reasons in Section~\ref{sec:rl_algorithmic_challenges}.
%
%is perhaps the single most important metric of CL performance. We recall that we tuned hyperparameters to maximize its value. PackNet is a clear winner, approaching $0.8$. Other methods perform significantly worse. A-GEM and Perfect Memory struggle, we conjecture possible explanations in Section \ref{sec:rl_algorithmic_challenges}.\piotrms{Final: This section is slightly awkward}%, but it would be more (?) awkward not to say anything about performance.}

\textbf{Forgetting} We observe that most CL methods are usually efficient in mitigating forgetting. However, we did not notice any boost when revisiting a task (see Figure~\ref{fig:training_graph}). Even if a different output head was employed, relearning the internal representation should have had an impact unless it changed considerably when revisiting the task. Additionally, we found A-GEM difficult to tune; consequently, with the best hyperparameter settings, it is relatively similar to the baseline  fine-tuning method (see details in Appendix \ref{sec:algorithmic_and_conceptual_challenges_appendix}). 


\textbf{Transfers} %The average forward transfer, as defined in \eqref{eq:forward_transfer}, for all methods and CW20 is summarized in Table \ref{tab:collected_resuls} and Appendix \ref{sec:forward_transfer_appendix} (Table \ref{tab:long_forward_transfer_table} and Figures \ref{fig:transfer_all}, \ref{fig:transfer_first_10}, \ref{fig:transfer_second_10}).
For all methods, forward transfer for the second ten tasks (and the same tasks are revisited) drops compared to the first ten tasks. This is in stark contrast to forgetting, which seems to be well under control. Among all methods, only fine-tuning and PackNet are able to achieve positive forward transfer ($0.20$ and $0.19$, resp.) as well as on the first ($0.32$ and $0.21$, resp.) and the second ($0.08$ and $0.17$, resp.) half of tasks. However, these are considerably smaller than $\text{RT}=0.46$, which in principle can even be exceeded, and which should be reached by a model that remembers all meaningful aspects of previously seen tasks, see \eqref{eq:forward_transfer_upperbound}. These results paint a fairly grim picture: we would expect improvement, rather than deterioration in performance, when revisiting previously seen tasks. There could be multiple reasons for this state of affairs. It could be attributed to the loss of plasticity,
similar to the effect observed in~\cite{DBLP:conf/nips/AshA20}.
%and a somewhat similar effect was observed in the context of supervised learning, see e.g., \cite{DBLP:conf/nips/AshA20}. 
Another reason could be related to the interference between CL mechanisms or setting and RL, for instance, hindering exploration. We did not observe any substantial cases of \textbf{backward transfer}, even though the benchmark is well suited to study this question due to the revisiting of tasks. See Appendix~\ref{sec:forgetting_appendix}.

%For details see Section \ref{sec:forward_transfer_appendix}. \piotrm{Forward transfers are rather unsatisfactory, especially for longer sequences.}
\begin{wrapfigure}{l}{0.70\linewidth}
    %\vskip -0.in
    \begin{center}
        \centerline{\includegraphics[width=0.7\columnwidth]{imgs/triplets.png}}
        \caption{\small \textbf{How forgetting impacts the forward transfer.} %The figure presents success rate throughout training on two sequences of three tasks. 
        Two different triplets of tasks learnt in sequence. An ideal agent learning on a sequence $A \rightarrow B \rightarrow C$ should have at least as good performance on task $C$ as an agent which just learns $A \rightarrow C$. In reality, an interfering task $B$ reduces this transfer, even when continual learning approaches are used.  % Right plot showcases that this effect appears even when learning on $A \rightarrow B \rightarrow A$.
        }
        \label{fig:triplets}
    \end{center}
    \vskip -0.3in
\end{wrapfigure}



\textbf{Triplets experiments} We illustrate how forgetting and forward transfer interact with each other in a simpler setting of three task sequences, see Figure~\ref{fig:triplets} and Appendix~\ref{sec:triplets_appendix}.
%Figure \ref{fig:triplets} thus shows a situation where remembering might be required to improve forward transfer and the overall training speed. 
We focus on sequences of tasks $A \rightarrow B \rightarrow C$, where $A \rightarrow C$ has significant positive forward transfer and $B \rightarrow C$ has a smaller or even negative transfer.
%
An efficient CL agent should be able to use information from $A$ to get good performance on $C$. However, interference introduced by $B$ reduces the final forward transfer (see Figure~\ref{fig:triplets}). The drive for reducing forgetting in CL agents has been primarily to perform well on previous tasks when we revisit them. With this example, we argue that an equally important reason to improve the memory of CL agents is to efficiently use past experiences to learn faster on new tasks. Currently, the tested CL methods often are not able to outperform the forgetful fine-tuning baseline. Observe that even the modularity-based PackNet approach struggles with this task. This possibly indicates that using the activation mask from task $B$ is enough to deteriorate the performance.

\textbf{PackNet} PackNet stands out in our evaluations.
We conjecture that developing related methods might be a promising research direction.
Besides further increasing performance, one could mitigate the limitations of PackNet.
%\michal{Replace last two sentences with: "However, it comes with a set of limitations; therefore we believe that developing less constrained related methods could be a promising research direction.}
PackNet relies on knowing task identity during evaluation. While this assumption is met in our benchmark, it is an interesting topic for future research to develop methods that cope without task identity. Another nuisance is that PackNet assigns some fixed fraction of parameters to a task. This necessitates knowledge of the length of the sequence in advance.
Additionally, when the second ten tasks of \cwtwenty{} start, PackNet performance degrades, showing its potentially inefficient use of capacity and past knowledge, given that the second ten tasks are identical with the first ten and hence no additional capacity is needed. %Finally, by construction PackNet does not allow backward transfer, though no other method had exhibited backward transfer either. 
In a broader context, we speculate that parameter isolation methods might be a promising direction towards better CL methods.

\textbf{Resources usage} In practical applications it is important to consider resources usage. All tested methods have relatively small overheads. For example, PackNet needs only $15\%$ more time than the baseline fine-tuning and it requires $50\%$ more neural network parameters (which is negligible when small networks like ours). See Appendix \ref{sec:resources_comparison} for details concerning other methods.

\textbf{Other observations} In stark contrast with the supervised learning setting, we found that replay based methods (Perfect Memory and A-GEM) suffer from poor performance. This is even though we allow for a generous replay, which could store the whole experience. Explaining and amending this situation is, in our view, an important research question. We conjecture that this happens due to the regularization of the critic network (which was unavoidable for these methods). We found multi-task learning attaining lower scores than PackNet, the best CL method and comparable to the second one, EWC. We think this suggests interesting research directions for multi-task learning.

% Finally, we refer the reader to Appendix~\ref{sec:cwtwenty_graph_and_analysis_appendix} for further analysis and ablation studies providing a more complete picture of the benchmark which for brevity constraints we could not fully convey here. % \razp{maybe re-edit but something of this sort at the end.}

\subsection{RL-Related Challenges}\label{sec:rl_algorithmic_challenges}

% \maciejws{Mźaybe we could move this to the beginning of this section, before the Forgetting paragraph?}
Reinforcement learning brings a set of issues not present in the supervised learning setting, e.g., exploration, varying reward scales, and stochasticity of environments. We argue that it is imperative to have a reliable benchmark to assess the efficiency of CL algorithms with respect to these problems. We find that some current methods are not well adjusted to the RL setting and require non-trivial conceptual considerations and careful tuning of hyperparameters, see details in Appendix~\ref{sec:algorithmic_and_conceptual_challenges_appendix}. 

An important design choice is whether or not to regularize the critic in the actor-critic framework (e.g. in SAC). We find it beneficial to focus on reducing forgetting in the actor while allowing the critic to freely adapt to the current task (note that critic is used only in training of the current task), similar to \cite{DBLP:conf/icml/Schwarz0LGTPH18}. %In fact, improvements offered by this approach are so significant that some of the tested methods are able to outperform the results obtained in the multi-task setting, where critic has to ''cover'' all tasks at the same time. 
% This is much different from the supervised setting, in which multi-task learning is often an upper bound to CL.
On the other hand, a forgetful critic is controversial. This can be sharply seen when the same task is repeated and the critic needs to learn from scratch. Additionally, not all methods can be trivially adapted to the 'actor-only regularization' setting, as for example replay based methods. In Appendix \ref{sec:algorithmic_and_conceptual_challenges_appendix} we examine these issues empirically, by showing experiments with critic regularization for EWC.

Another aspect is the exploration and its non-trivial impact on transfers. As it was observed, transfers from a given task to the same one are sometimes poor. We show in Appendix \ref{sec:diagonal_transfers_appendix} that this results from the fact that at the task change the replay buffer is emptied and SAC collects new samples from scratch, usually by using the uniform policy. Learning on these random samples reduces performance on the current task and thus the forward transfer. Experimentally, we find that  not resetting the buffer or using the current policy for exploration improves the transfer on the diagonal. % At the same time, it could lead to d off-diagonal~transfers.  %\maciejw{Additional point: the samples are (extremely) off-policy}


==> 609bc59dc39be977132478d8 copy/experiments_old_28_01.tex <==

Main experimental takeaways discussion
\begin{itemize}
    \item Forgetting seems mainly to be mitigated by existing methods.
    \item Methods tend to transfer poorly - lack of transfer between tasks seems embarrassing to the field.
    \item Methods saturate on longer sequences.
\end{itemize}

\maciejw{I wonder if these takeaways aren't too much connected to the hyperparameters we have chosen. For example, if we used smaller regularization coefficient for EWC then it would have better transfer and more forgetting. On the other hand, we chose these hyperparameters by looking at the thing that most people look at in CL - the average performance at the end of the training. So maybe we could argue that focusing on that in some sense discourages people from caring about forward transfer? 2021-01-27}

In our experiments, we pose the following research questions: what is the level of the forward transfer and forgetting in robotic tasks without using CL methods? How do CL methods change this picture? More specifically, is forgetting helpful or harmful for forward transfer? Further, we ask how much information about pairs and triples could be beneficial for longer sequences.

\piotrm{We should state take-aways and also put them in the intro.}


\subsection{\benchmark{} experiments}
Ideas:
\begin{enumerate}
    \item Present value at the end of ten tasks (i.e. the right most one on Figure \ref{fig:training_graph}) as on of main matric.
    \item Have it for all CL methods.
    \item Present value at the end of twenty tasks as the second main metric.
    \item Calculate forgetting -- \razp{I'm ashamed to say I'm not even sure what people tend to report usually. I tend to only look at learning curves and make "qualitative" observations. I think Arslan had proposed something on one of his paper that seemed relatively popular; but I think is exactly point (1) which is the performance at the end on all previous tasks. I think in progressive nets paper we had a nice table where we colored with green vs blue and basically was looking at the performance of training each task ? or was it some AUC as well. Someone should open that paper :) }(is it the classical thing to do?).
\end{enumerate}

\subsection{Pair experiments}
Ideas:

\begin{enumerate}
    \item Present the forward transfer matrices. Here probably a subset in the appendix the whole table
    \item Describe some stories behind:  various relations, @PM mockup
    \item Why we do not say anything about forgetting here? nice-to-have \razp{ There are some thoughts here. re: catastrophic forgetting. We will be measuring it. Would be nice to plot catastrophic forgetting vs forward transfer to see if there is some structure there (with respect to methods). The other thing is recovering of the forgotten policies. So if we have the sequence of 20 tasks where we revisit tasks. It would be nice here to see if there is a correlation between how much you remember the previous task and how quickly you recover it. }
    \item upper-bound
          \kucil{2021-01-22: transfer with significance correction. Also in the Appendix table with CIs}
\end{enumerate}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/heatmap_transfer.png}}%pair_plot_mockup.png}}
        \caption{\piotrm{todo please put the final version with desscription.} }\label{fig:transfer_matrix_haatmmap}
    \end{center}
    \vskip -0.2in
\end{figure}

% \begin{figure}[ht]
%     \vskip 0.2in
%     \begin{center}
%     \centerline{\includegraphics[width=\columnwidth]{imgs/transfer_heatmap_significant.png}}%pair_plot_mockup.png}}
%     \caption{fillme (significance correction). atm for comparison. (todo: put normalized)}
%     \end{center}
%     \vskip -0.2in
% \end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \subfigure[A $\rightarrow$ B $\rightarrow$ C]{
            \includegraphics[width=0.47\columnwidth]{imgs/triple.png}
        }
        \subfigure[A $\rightarrow$ B $\rightarrow$ A]{
            \includegraphics[width=0.47\columnwidth]{imgs/triple_to_self.png}
        }
        \caption{\textbf{How forgetting impacts the forward transfer.} Figures present performance on task C with different types of pretraining. (a) A $\rightarrow$ C has very positive transfer, but putting a destructive task B between them causes the model to forget useful knowledge from task A. (b) This effect appears even if we consider transfers to itself, i.e A $\rightarrow$ B $\rightarrow$ A.}
    \end{center}
    \vskip -0.2in
\end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/positive_transfer_graph_example.png}}
        \caption{\textbf{Cherry pick with positive transfer}.}
    \end{center}
    \vskip -0.2in
\end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/negative_transfer_example.png}}
        \caption{\textbf{Cherry pick with negative transfer transfer}.}
    \end{center}
    \vskip -0.2in
\end{figure}

Detailed tables and graphs are presented in Section \ref{sec:pair_experiments_appendix}.

\subsection{Triples experiments}

\begin{itemize}
    \item Possibly run progressive nets as baseline.
\end{itemize}

\section{Random observations/notes}
\begin{itemize}
    \item \maciejw{Many algorithms didn't work as it is (e.g. EWC required deriving Fisher with some non-obvious assumptions). I know that RL aspects are not really our focus, but maybe we could have a paragraph somewhere where we say that there were some issues and refer the reader to the appendix for details?} This is RL specific.
    \item \maciejw{Continual learning methods perform much better when they do not regularize the critic, on the other hand it may be difficult to use them for retraining.}
    \item \maciejw{Experience replay methods, although they excel in supervised setting, do not perform very well in our benchmark. It maybe partly because they are forced to regularize the critic as well as the actor.}
    \item \maciejw{It seems that transfer from a task to itself is usually not as good as we would expect -- maybe because there is too much noise at the beginning of the training?}
    \item \michal{when we consider CL methods, transfer is diminished compared to vanilla, EXCEPT FOR PackNet. TODO: compare to "upper bound"}

    \item \michal{when the sequence of tasks is repeated, performance is surprisingly poor on second half - why?}
    \item \michal{Regarding poor "transfer" from X to X: at some point we observed that even just resetting the buffer after first "instance" of the same task leads to poor transfer metric. We'd need to double-check though}

    \item \piotrm{We observe little forgetting for any method but vanilla. See Figure \ref{fig:forgetting}} Than it would follow that methods are better because of transfers?
    \item \piotrm{We possibly need to justify the selection of $1$M steps more carefully, as the curves are still growing. See Figure \ref{fig:long_sequence}}
    \item \michal{In the current version (task set), MTL performs at the level of EWC and worse than PackNet -- should we worry?}
\end{itemize}

To do list:
\begin{itemize}
    \item For above see if there are some correlations @all
\end{itemize}
To do list (nice to have):
\begin{itemize}
    \item Multi-task learning with separate critics
    \item Find examples of backward transfer
    \item Run experiment without multi-head (possibly with task\_id instead)
    \item Put a case study forgetting vs transfer (e.g. "L2 hps analysis" done by Maciek)
    \item Possibly mention (or compute if relevant) 'transfer score' of progressive nets.
\end{itemize}

==> 609bc59dc39be977132478d8 copy/fisher_derivation.tex <==
\begin{proof} We fix parameters $\theta_0$, denote $\mu_{0} = \mu(\theta_0),\sigma_{0} = \sigma(\theta_0)$ and $\mathcal{N}_{0}:=\mathcal{N}_{0}(\mu_{0},\sigma_{0}^{2})$. We will calculate the the diagonal Fisher matrix coefficient at $\theta_0$ using the fact that it is the curvature of the  Kullback–Leibler divergence:
    \begin{equation} \label{eq:dkl_curvature}
        \mathcal{I}_{kk} = \frac{\partial^2 }{\partial \theta_k^2} F(\theta), \quad F(\theta) := f(\mu(\theta_{i}),\sigma(\theta_{i})),
    \end{equation}
    where
    \[
        f(\mu,\sigma):={\displaystyle D_{\text{KL}}\big({\mathcal{N}}_{0}\parallel{\mathcal{N}}(\mu, \sigma^2)\big)=\frac{1}{2}\left\{ \left({\frac{\sigma_{0}}{\sigma}}\right)^{2}+{\frac{(\mu-\mu_{0})^{2}}{\sigma^{2}}}-1+2\ln\frac{\sigma}{\sigma_{0}}\right\} }.
    \]
    We start with
    \begin{equation}
        \frac{\partial f}{\partial\mu}=\frac{(\mu-\mu_{0})}{\sigma^{2}},\quad\text{thus}\quad\frac{\partial f}{\partial\mu}(\mu_{0},\sigma_{0})=0.\label{eq:dmu}
    \end{equation}
    Further
    \begin{equation}
        \frac{\partial^{2}f}{\partial\mu^{2}}=\frac{1}{\sigma^{2}},\quad\text{thus}\quad\frac{\partial f}{\partial\mu}(\mu_{0},\sigma_{0})=\frac{1}{\sigma_{0}^{2}}.\label{eq:d2mu}
    \end{equation}
    For $\sigma$ we have
    % \begin{equation}
    %     \frac{\partial f}{\partial\sigma}=\frac{1}{2}\left\{ -2\frac{\sigma_{0}^{2}}{\sigma^{3}}-2\frac{(\mu-\mu_{0})^{2}}{\sigma^{3}}+\frac{2}{\sigma}\right\} =-\frac{\sigma_{0}^{2}}{\sigma^{3}}-\frac{(\mu-\mu_{0})^{2}}{\sigma^{3}}+\frac{1}{\sigma},\quad\text{thus}\quad\frac{\partial f}{\partial\sigma}(\mu_{0},\sigma_{0})=-\frac{\sigma_{0}^{2}}{\sigma_{0}^{3}}-\frac{0}{\sigma^{3}}+\frac{1}{\sigma_{0}}=0.
    % \end{equation}
    \begin{align}\label{eq:dsigma}
        &\frac{\partial f}{\partial\sigma}=\frac{1}{2}\left\{ -2\frac{\sigma_{0}^{2}}{\sigma^{3}}-2\frac{(\mu-\mu_{0})^{2}}{\sigma^{3}}+\frac{2}{\sigma}\right\} =-\frac{\sigma_{0}^{2}}{\sigma^{3}}-\frac{(\mu-\mu_{0})^{2}}{\sigma^{3}}+\frac{1}{\sigma},\\
        &\frac{\partial f}{\partial\sigma}(\mu_{0},\sigma_{0})=-\frac{\sigma_{0}^{2}}{\sigma_{0}^{3}}-\frac{0}{\sigma^{3}}+\frac{1}{\sigma_{0}}=0.\nonumber
    \end{align}
    Further
    \begin{equation}
        \frac{\partial^{2}f}{\partial\sigma^{2}}=3\frac{\sigma_{0}^{2}}{\sigma^{4}}+3\frac{(\mu-\mu_{0})^{2}}{\sigma^{4}}-\frac{1}{\sigma^{2}},\quad\text{thus}\quad\frac{\partial^{2}f}{\partial\sigma^{2}}(\mu_{0},\sigma_{0})=3\frac{\sigma_{0}^{2}}{\sigma_{0}^{4}}+3\frac{0}{\sigma^{4}}-\frac{1}{\sigma_{0}^{2}}=\frac{2}{\sigma_{0}^{2}}.\label{eq:d2sigma}
    \end{equation}
    Now, we come back to \eqref{eq:dkl_curvature}. Applying the chain rule
    \[
        \frac{\partial^2 F}{\partial \theta_k^2} =
        \frac{\partial^2 \mu}{\partial \theta_k^2}\cdot\frac{\partial f}{\partial\mu}+
        \left(\frac{\partial \mu}{\partial \theta_k}\right)^2\cdot\frac{\partial^2 f}{\partial\mu^2}+
        \frac{\partial^2 \sigma}{\partial \theta_k^2}\cdot\frac{\partial f}{\partial\sigma}+
        \left(\frac{\partial \sigma}{\partial \theta_k}\right)\cdot\frac{\partial^2 f}{\partial\sigma^2}.
    \]
    When evaluating at $\theta = \theta_0$ the first and third terms vanish, by \eqref{eq:dmu} and \eqref{eq:dsigma}. Thus
    \[
        \frac{\partial^2 F}{\partial \theta_k^2}(\theta_0) =
        \left(\frac{\partial \mu}{\partial \theta_k}(\theta_0)\right)^2\cdot\frac{\partial^2 f}{\partial\mu^2}(\theta_0)+
        \left(\frac{\partial \sigma}{\partial \theta_k}(\theta_0)\right)^2\cdot\frac{\partial^2 f}{\partial\sigma^2}(\theta_0).
    \]
    Now we use (\ref{eq:dsigma}) and (\ref{eq:d2sigma}) we arrive at \eqref{eq:fisher_diagonal}.
    % \[
    %     \frac{\partial^2 F}{\partial \theta_k^2}(\theta_0) =
    %     \left(\frac{\partial \mu}{\partial \theta_k}(\theta_0)\cdot\frac{1}{\sigma(\theta^{0})}\right)^{2}+
    %     2\left(\frac{\partial \sigma}{\partial \theta_k}(\theta_0)\cdot\frac{1}{\sigma(\theta^{0})}\right)^{2}.
    % \]

\end{proof}
% By the chain rule we have
% \[
%     F'(\theta_{i})=\mu'(\theta_{i})\frac{\partial f}{\partial\mu}+\sigma'(\theta_{i})\frac{\partial f}{\partial\sigma}.
% \]
% Thus at $\theta_{i}^{0}$ we get (we use (\ref{eq:dmu}) and (\ref{eq:dsigma}))
% \[
%     F'(\theta_{i}^{0})=\mu'(\theta_{i}^{0})\frac{\partial f}{\partial\mu}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)+\sigma'(\theta_{i}^{0})\frac{\partial f}{\partial\sigma}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)=0.
% \]
% For the second derivative we have
% \[
%     F''(\theta_{i})=\mu''(\theta_{i})\frac{\partial f}{\partial\mu}+\left(\mu'(\theta_{i})\right)^{2}\frac{\partial^{2}f}{\partial\mu^{2}}+\sigma''(\theta_{i})\frac{\partial f}{\partial\sigma}+\left(\sigma'(\theta_{i})\right)^{2}\frac{\partial^{2}f}{\partial\sigma^{2}}.
% \]
% Let us evaluate at $\theta_{i}^{0}$
% \begin{align*}
%     F''(\theta_{i}^{0})= & \mu''(\theta_{i}^{0})\frac{\partial f}{\partial\mu}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)+\left(\mu'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial\mu^{2}}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)               \\
%                          & +\sigma''(\theta_{i}^{0})\frac{\partial f}{\partial\sigma}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)+\left(\sigma'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial\sigma^{2}}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right).
% \end{align*}
% By (\ref{eq:dmu}) and (\ref{eq:dsigma}) the first and third terms
% disappear.
% \[
%     F''(\theta_{i}^{0})=\left(\mu'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial\mu^{2}}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right)+\left(\sigma'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial\sigma^{2}}\left(\mu(\theta_{i}^{0}),\sigma(\theta_{i}^{0})\right).
% \]
% Now we use (\ref{eq:dsigma}) and (\ref{eq:d2sigma}) we arrive at
% \[
%     F''(\theta_{i}^{0})=\left(\frac{\mu'(\theta_{i}^{0})}{\sigma(\theta_{i}^{0})}\right)^{2}+2\left(\frac{\sigma'(\theta_{i}^{0})}{\sigma(\theta_{i}^{0})}\right)^{2}.
% \]

% We can also parametrize with $\sigma^{2}$. For clarity we will use
% $s=\sigma^{2}$ ($s_{0}=\sigma_{0}^{2})$. Then
% \[
%     f(\mu,s)={\displaystyle D_{\text{KL}}({\mathcal{N}}_{0}\parallel{\mathcal{N}}_{1})=\frac{1}{2}\left\{ {\frac{\sigma_{0}^{2}}{s}}+{\frac{(\mu-\mu_{0})^{2}}{s}}-1+\ln\frac{s}{\sigma_{0}^{2}}\right\} }.
% \]
% Derivative with respect to $s$ is
% \[
%     \frac{\partial f}{\partial s}=\frac{1}{2}\left\{ -{\frac{\sigma_{0}^{2}}{s^{2}}}-{\frac{(\mu-\mu_{0})^{2}}{s^{2}}}+\frac{1}{s}\right\} ,\quad\text{thus}\quad\frac{\partial f}{\partial s}(\mu_{0},\sigma_{0}^{2})=\frac{1}{2}\left\{ -{\frac{\sigma_{0}^{2}}{\sigma_{0}^{4}}}-{\frac{0}{s_{0}^{2}}}+\frac{1}{\sigma_{0}^{2}}\right\} =0.
% \]
% And the second derivative
% \[
%     \frac{\partial f}{\partial s}=\frac{1}{2}\left\{ 2\frac{\sigma_{0}^{2}}{s^{3}}+2\frac{(\mu-\mu_{0})^{2}}{s^{3}}-\frac{1}{s^{2}}\right\} ,\quad\text{thus}\quad\frac{\partial f}{\partial s}(\mu_{0},\sigma_{0}^{2})=\frac{1}{2}\left\{ 2\frac{\sigma_{0}^{2}}{\sigma_{0}^{6}}+2\frac{0}{s_{0}^{6}}-\frac{1}{\sigma_{0}^{4}}\right\} =\frac{1}{2\sigma_{0}^{4}}.
% \]
% Analogous calculations led to
% \begin{align*}
%     F''(\theta_{i})= & \mu''(\theta_{i})\frac{\partial f}{\partial\mu}+\left(\mu'(\theta_{i})\right)^{2}\frac{\partial^{2}f}{\partial\mu^{2}}     \\
%                      & +s''(\theta_{i})\frac{\partial f}{\partial\sigma}+\left(s'(\theta_{i})\right)^{2}\frac{\partial^{2}f}{\partial\sigma^{2}},
% \end{align*}
% and
% \[
%     F''(\theta_{i}^{0})=\left(\mu'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial\mu^{2}}\left(\mu(\theta_{i}^{0}),s(\theta_{i}^{0})\right)+\left(s'(\theta_{i}^{0})\right)^{2}\frac{\partial^{2}f}{\partial s^{2}}\left(\mu(\theta_{i}^{0}),s(\theta_{i}^{0})\right).
% \]
% \[
%     F''(\theta_{i}^{0})=\left(\frac{\mu'(\theta_{i}^{0})}{\sigma(\theta_{i}^{0})}\right)^{2}+\frac{1}{2}\left(\frac{s'(\theta_{i}^{0})}{\sigma^{2}(\theta_{i}^{0})}\right)^{2}.
% \]


% \subsubsection{Multivariate case}

% For multidimensional normal distributions:

% \[
%     f(\mu,\sigma)={\displaystyle D_{\text{KL}}({\mathcal{N}}_{0}\parallel{\mathcal{N}}_{1}}) = \frac{1}{2}\left[\log\frac{|S|}{|S_0|} - d + \text{tr} \{ S^{-1}S_0 \} + (\mu - \mu_0)^T S^{-1}(\mu - \mu_0)\right].
% \]

% Assuming that the covariance matrix is diagonal with $S^{jj} = (\sigma^j)^2$:

% \begin{equation}
%     \begin{split}
%         {\displaystyle D_{\text{KL}}({\mathcal{N}}_{0}\parallel{\mathcal{N}}_{1}}) &= \frac{1}{2}\left[\log \Pi_j \frac{ (\sigma^j)^2}{(\sigma_0^j)^2} - d + \sum_j \frac{(\sigma_0^j)^2}{(\sigma^j)^2} + \sum_j \frac{(\mu^j - \mu^j_0)^2}{(\sigma^j)^2}\right] \\
%         & = \frac{1}{2}\left[2\sum_j \log  \frac{\sigma^j}{\sigma_0^j} - d + \sum_j \frac{(\sigma_0^j)^2}{(\sigma^j)^2} + \sum_j \frac{(\mu^j - \mu^j_0)^2}{(\sigma^j)^2}\right] \\
%         & = \sum_j \frac{1}{2}\left[ \left(\frac{\sigma_0^j}{\sigma^j}\right)^2 + \frac{(\mu^j - \mu^j_0)^2}{(\sigma^j)^2} - 1 + 2\log  \frac{\sigma^j}{\sigma_0^j} \right].
%     \end{split}
% \end{equation}

% Thus each dimension can be calculated separately using the derivation from the previous section and then summed up.


==> 609bc59dc39be977132478d8 copy/forgetting_qualitiatie_analysis.tex <==
\subsubsection{Vanilla and AGEM} The forgetting occurs quickly after the training of a given task has finished, see Figure \ref{fig:forgetting_agem} for AGEM, results for the vanilla method are similar. 


\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=agem_pm_zeroed.png}}
    \caption{Forgetting plot for AGEM (we zero the plot until the task ends)} \label{fig:forgetting_agem}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{EWC} For EWC the forgetting is rather small with the exception of the first task, which decreases quickly after its training has completed, see Figure \ref{fig:forgetting_ewc}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=ewc_pm_zeroed.png}}
    \caption{Forgetting plot for EWC (we zero the plot until the task ends)} \label{fig:forgetting_ewc}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{MAS} MAS experiences mild forgetting shortly after a given task has completed, see Figure \ref{fig:forgetting_mas}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=mas_pm_zeroed.png}}
    \caption{Forgetting plot for MAS (we zero the plot until the task ends)} \label{fig:forgetting_mas}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{Packnet} See Figure \ref{fig:forgetting_packnet} (note that some variations are due to noise).
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=packnet_pm_zeroed.png}}
    \caption{Forgetting plot for packnet (we zero the plot until the task ends)} \label{fig:forgetting_packnet}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{VCL} VCL behaves relatively worse than other methods. We can observe small decrease over the whole training, see Figure \ref{fig:forgetting_vlc}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=vcl_pm_zeroed.png}}
    \caption{Forgetting plot for VCL (we zero the plot until the task ends)} \label{fig:forgetting_vlc}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{L2} L2 is surprisingly good taking into account it simplicity. We observe, however, an erratic drops in performace in a 'random' moments. We conjecture that these are when conflicting information appears. See Figure \ref{fig:forgetting_l2}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=l2_pm_zeroed.png}}
    \caption{Forgetting plot for L2 (we zero the plot until the task ends)} \label{fig:forgetting_l2}
    \end{center}
    \vskip -0.2in
\end{figure*}

==> 609bc59dc39be977132478d8 copy/forgetting_table.tex <==
\begin{table}[h!]
    \begin{center}
        \begin{tabular}{lrrrrrrrrrr}
            \toprule
            {} &  \rotatebox[origin=c]{90}{hammer-v1} &  \rotatebox[origin=c]{90}{push-wall-v1} &  \rotatebox[origin=c]{90}{faucet-close-v1} &  \rotatebox[origin=c]{90}{push-back-v1} &  \rotatebox[origin=c]{90}{stick-pull-v1} &  \rotatebox[origin=c]{90}{handle-press-side-v1} &  \rotatebox[origin=c]{90}{push-v1} &  \rotatebox[origin=c]{90}{shelf-place-v1} &  \rotatebox[origin=c]{90}{window-close-v1} &  \rotatebox[origin=c]{90}{peg-unplug-side-v1} \\
            cl\_method &                                      &                                         &                                            &                                         &                                          &                                                 &                                    &                                           &                                            &                                               \\
            \midrule
            None      &                                 0.89 &                                    0.72 &                                       0.95 &                                    0.99 &                                     0.68 &                                            0.96 &                               0.83 &                                      0.45 &                                       0.82 &                                          0.00 \\
            agem      &                                 0.88 &                                    0.72 &                                       0.86 &                                    0.90 &                                     0.75 &                                            0.86 &                               0.78 &                                      0.84 &                                       0.76 &                                          0.00 \\
            ewc       &                                 0.38 &                                    0.13 &                                       0.05 &                                    0.03 &                                    -0.11 &                                           -0.06 &                              -0.01 &                                     -0.00 &                                       0.02 &                                          0.00 \\
            l2        &                                 0.14 &                                    0.06 &                                       0.14 &                                    0.00 &                                    -0.02 &                                            0.01 &                               0.05 &                                     -0.01 &                                      -0.02 &                                          0.00 \\
            mas       &                                 0.01 &                                    0.03 &                                       0.05 &                                   -0.02 &                                    -0.14 &                                           -0.08 &                              -0.00 &                                      0.02 &                                      -0.01 &                                          0.00 \\
            packnet   &                                -0.07 &                                    0.07 &                                       0.00 &                                    0.00 &                                    -0.00 &                                            0.00 &                               0.04 &                                     -0.00 &                                      -0.03 &                                          0.00 \\
            vcl       &                                 0.17 &                                    0.15 &                                       0.20 &                                    0.15 &                                     0.09 &                                            0.43 &                               0.11 &                                      0.07 &                                       0.13 &                                          0.00 \\
            \bottomrule
        \end{tabular}
        
        \caption{Averages over forgetting.} \label{tab:forgetting_table}
    \end{center}
\end{table}

==> 609bc59dc39be977132478d8 copy/long_transfer_tables.tex <==
\begin{table}
\centering
\caption{Summary of FT experiments}
\begin{tabular}{lllllll}
\toprule
identifier &                    FT &          FT\_first\_ten &         FT\_second\_ten &         Normalized FT & Normalized FT\_first\_ten & CI\_second\_half\_normalized\_ft \\
\midrule
      None &     0.07 [0.06, 0.09] &     0.12 [0.11, 0.14] &     0.03 [0.00, 0.05] &     0.20 [0.17, 0.23] &       0.32 [0.29, 0.35] &            0.08 [0.04, 0.13] \\
       ewc &  -0.07 [-0.09, -0.05] &    0.01 [-0.02, 0.03] &  -0.14 [-0.17, -0.11] &  -0.19 [-0.25, -0.13] &      0.02 [-0.05, 0.07] &         -0.39 [-0.49, -0.30] \\
        l2 &  -0.25 [-0.29, -0.22] &  -0.21 [-0.25, -0.17] &  -0.30 [-0.33, -0.27] &  -0.75 [-0.87, -0.64] &    -0.64 [-0.77, -0.52] &         -0.86 [-0.97, -0.75] \\
       mas &  -0.19 [-0.20, -0.17] &  -0.13 [-0.15, -0.11] &  -0.24 [-0.27, -0.22] &  -0.52 [-0.58, -0.47] &    -0.36 [-0.42, -0.30] &         -0.68 [-0.77, -0.61] \\
   packnet &     0.07 [0.06, 0.09] &     0.10 [0.08, 0.11] &     0.05 [0.03, 0.07] &     0.18 [0.14, 0.22] &       0.22 [0.17, 0.27] &            0.14 [0.09, 0.19] \\
\bottomrule
\end{tabular}\label{tab:long_forward_transfer_table}
\end{table}

%\begin{table}
%\centering
%\caption{Summary of FT experiments}
%\label{tab:long_forward_transfer_table}
%\begin{tabular}{lrrrrrr}
%\toprule
%identifier &    FT &  FT\_first\_ten &  FT\_second\_ten &  Normalized FT &  Normalized FT\_first\_ten &  Normalized FT\_second\_ten \\
%\midrule
%      None &  0.08 &          0.13 &           0.04 &           0.22 &                     0.33 &                      0.10 \\
%       ewc & -0.05 &          0.02 &          -0.13 &          -0.13 &                     0.08 &                     -0.33 \\
%        l2 & -0.23 &         -0.20 &          -0.27 &          -0.69 &                    -0.61 &                     -0.77 \\
%       mas & -0.18 &         -0.13 &          -0.22 &          -0.49 &                    -0.36 &                     -0.62 \\
%   packnet &  0.04 &          0.16 &          -0.08 &           0.05 &                     0.38 &                     -0.28 \\
%\bottomrule
%\end{tabular}
%\end{table}


\begin{table}[ht]
\centering
\caption{Normalized Forward Transfer, first ten tasks}
\begin{tabular}{lllllllllll}
\toprule
train/active\_env &                     0 &                     1 &                    2 &                     3 &                     4 &                     5 &                     6 &                     7 &                     8 &                     9 \\
identifier &                       &                       &                      &                       &                       &                       &                       &                       &                       &                       \\
\midrule
None       &     0.13 [0.05, 0.20] &    0.06 [-0.08, 0.19] &    0.39 [0.24, 0.51] &     0.76 [0.73, 0.79] &    0.08 [-0.05, 0.20] &     0.55 [0.50, 0.59] &   -0.11 [-0.24, 0.01] &     0.13 [0.04, 0.22] &     0.44 [0.38, 0.50] &     0.77 [0.70, 0.81] \\
ewc        &     0.13 [0.05, 0.20] &  -0.10 [-0.19, -0.02] &    0.35 [0.20, 0.49] &     0.66 [0.51, 0.76] &  -0.36 [-0.45, -0.27] &     0.14 [0.03, 0.25] &  -0.81 [-0.98, -0.63] &  -0.10 [-0.19, -0.01] &     0.35 [0.22, 0.47] &   -0.11 [-0.63, 0.32] \\
l2         &     0.14 [0.07, 0.21] &  -0.39 [-0.52, -0.25] &  -0.09 [-0.40, 0.20] &  -0.26 [-0.52, -0.01] &  -0.45 [-0.52, -0.39] &  -1.84 [-2.42, -1.28] &  -1.69 [-1.93, -1.44] &  -0.20 [-0.26, -0.15] &  -0.91 [-1.46, -0.37] &  -0.68 [-1.21, -0.25] \\
mas        &     0.13 [0.05, 0.20] &  -0.63 [-0.72, -0.53] &   0.04 [-0.20, 0.24] &   -0.09 [-0.31, 0.12] &  -0.35 [-0.45, -0.25] &  -0.44 [-0.59, -0.30] &  -1.38 [-1.60, -1.17] &  -0.18 [-0.25, -0.12] &   -0.18 [-0.56, 0.14] &  -0.51 [-1.06, -0.04] \\
packnet    &  -0.49 [-0.65, -0.35] &   -0.08 [-0.19, 0.02] &    0.33 [0.09, 0.50] &     0.80 [0.76, 0.83] &  -0.21 [-0.33, -0.09] &    0.05 [-0.22, 0.29] &     0.12 [0.04, 0.20] &     0.44 [0.34, 0.53] &     0.45 [0.28, 0.58] &     0.80 [0.72, 0.86] \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[ht]
\centering
\caption{Normalized Forward Transfer, second ten tasks}
\begin{tabular}{lllllllllll}
\toprule
train/active\_env &                    10 &                    11 &                    12 &                    13 &                    14 &                    15 &                    16 &                    17 &                    18 &                    19 \\
identifier &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       \\
\midrule
None       &   -0.30 [-0.62, 0.00] &  -0.21 [-0.30, -0.12] &    0.04 [-0.13, 0.20] &     0.53 [0.44, 0.60] &  -0.19 [-0.31, -0.05] &     0.48 [0.41, 0.56] &  -0.79 [-0.96, -0.63] &    0.02 [-0.07, 0.11] &     0.52 [0.45, 0.59] &     0.73 [0.66, 0.78] \\
ewc        &  -0.66 [-0.97, -0.37] &  -0.57 [-0.70, -0.45] &  -0.36 [-0.67, -0.07] &     0.39 [0.25, 0.51] &  -0.47 [-0.53, -0.41] &    0.03 [-0.13, 0.19] &  -1.83 [-2.06, -1.60] &  -0.20 [-0.27, -0.13] &   -0.06 [-0.45, 0.28] &   -0.16 [-0.72, 0.29] \\
l2         &  -0.49 [-0.82, -0.16] &  -0.77 [-0.90, -0.65] &  -0.74 [-1.11, -0.42] &  -0.59 [-0.79, -0.41] &  -0.49 [-0.55, -0.43] &  -1.52 [-1.99, -1.08] &  -2.44 [-2.64, -2.25] &  -0.23 [-0.29, -0.18] &  -0.74 [-1.21, -0.29] &  -0.59 [-1.09, -0.18] \\
mas        &  -0.41 [-0.76, -0.09] &  -0.71 [-0.81, -0.61] &  -0.67 [-1.00, -0.38] &  -0.33 [-0.55, -0.13] &  -0.45 [-0.53, -0.37] &  -1.05 [-1.40, -0.72] &  -2.07 [-2.29, -1.85] &  -0.22 [-0.28, -0.17] &  -0.67 [-1.18, -0.18] &   -0.26 [-0.73, 0.14] \\
packnet    &  -0.41 [-0.74, -0.10] &    0.08 [-0.02, 0.17] &     0.42 [0.31, 0.50] &     0.82 [0.79, 0.85] &  -0.24 [-0.35, -0.13] &    0.17 [-0.00, 0.34] &  -0.34 [-0.47, -0.19] &   -0.03 [-0.12, 0.06] &     0.44 [0.28, 0.58] &     0.46 [0.14, 0.70] \\
\bottomrule
\end{tabular}
\end{table}



%\begin{table}[ht]
%\centering
%\caption{Normalized Forward Transfer, first ten tasks}
%\begin{tabular}{lp{1.5cm}rrrrrrrrr}
%\toprule
%train/active\_env &     0 &     1 &     2 &     3 &     4 &     5 &     6 &     7 &     8 &     9 \\
%identifier &       &       &       &       &       &       &       &       &       &       \\
%\midrule
%None       &  0.13 [0.11, 0.12] &  0.06 &  0.46 &  0.77 &  0.09 &  0.58 & -0.05 &  0.08 &  0.47 &  0.77 \\
%ewc        &  0.13 & -0.02 &  0.44 &  0.53 & -0.32 &  0.15 & -0.93 & -0.10 &  0.40 &  0.48 \\
%l2         &  0.11 & -0.30 &  0.00 & -0.23 & -0.43 & -1.68 & -1.82 & -0.19 & -0.64 & -0.87 \\
%mas        &  0.13 & -0.60 &  0.23 & -0.12 & -0.34 & -0.53 & -1.40 & -0.19 & -0.10 & -0.68 \\
%packnet    & -0.14 &  0.17 &  0.59 &  0.84 &  0.04 &  0.56 &  0.06 &  0.36 &  0.57 &  0.81 \\
%\bottomrule
%\end{tabular}
%\end{table}
%
%\begin{table}[ht]
%\centering
%\caption{Normalized Forward Transfer, second ten tasks}
%\begin{tabular}{lrrrrrrrrrr}
%\toprule
%train/active\_env &    10 &    11 &    12 &    13 &    14 &    15 &    16 &    17 &    18 &    19 \\
%identifier &       &       &       &       &       &       &       &       &       &       \\
%\midrule
%None       & -0.36 & -0.17 &  0.06 &  0.55 & -0.16 &  0.46 & -0.72 &  0.13 &  0.55 &  0.71 \\
%ewc        & -0.80 & -0.57 & -0.36 &  0.38 & -0.49 &  0.09 & -1.94 & -0.15 &  0.27 &  0.27 \\
%l2         & -0.31 & -0.87 & -0.62 & -0.41 & -0.49 & -1.15 & -2.62 & -0.23 & -0.75 & -0.29 \\
%mas        & -0.40 & -0.65 & -0.74 & -0.24 & -0.42 & -0.79 & -2.21 & -0.21 & -0.34 & -0.19 \\
%packnet    & -0.11 & -0.07 &  0.26 &  0.69 & -0.40 &  0.09 & -0.64 & -0.18 & -0.18 & -2.27 \\
%\bottomrule
%\end{tabular}
%\end{table}

==> 609bc59dc39be977132478d8 copy/mutli_task.tex <==
In multi-task experiments, we train $10$ tasks from CW10 simultaneously (we do not duplicate tasks as it is done in CW20). In our experiments, PopArt reward normalization~\cite{DBLP:conf/aaai/HesselSE0SH19} yields significant improvements ($0.66$ vs $0.50$ for the standard version, see also the top graph in  Figure~\ref{sec:average_success_big}). We observe that EWC and PackNet achieve results similar or better to multi-task learning. We consider this to be an interesting research direction. We conjecture that CL methods might benefit from the fact that the critic network stores only one value function (corresponding to the current task), see also discussion in Section \ref{sec:critic_regularizaiton_appendix}.

For multi-task training, we tested the following hyperparameter values: $\text{batch size} \in \{ 128, 256, 512 \}$ (selected value $=128$), $\text{learning rate} \in \{ \num{3e-5}, \num{1e-4}, \num{3e-4}, \num{1e-3} \}$ (selected value $=\num{1e-4}$).

==> 609bc59dc39be977132478d8 copy/pairs_vanilla_table.tex <==
\textbf{PM: this is now 15.01 a mock-up}

\begin{tabular}{lrrrrrrrrrr}
\toprule
task &  \rotatebox[origin=c]{90}{faucet-close-v1} &  \rotatebox[origin=c]{90}{hammer-v1} &  \rotatebox[origin=c]{90}{handle-press-side-v1} &  \rotatebox[origin=c]{90}{peg-unplug-side-v1} &  \rotatebox[origin=c]{90}{push-back-v1} &  \rotatebox[origin=c]{90}{push-v1} &  \rotatebox[origin=c]{90}{push-wall-v1} &  \rotatebox[origin=c]{90}{shelf-place-v1} &  \rotatebox[origin=c]{90}{stick-pull-v1} &  \rotatebox[origin=c]{90}{window-close-v1} \\
first\_task           &                  &            &                       &                     &               &          &               &                 &                &                  \\
\midrule
faucet-close-v1      &            0.182 &      0.015 &                 0.061 &               0.224 &         0.421 &   -0.043 &        -0.012 &           0.257 &          0.007 &            0.072 \\
hammer-v1            &            0.230 &      0.154 &                 0.112 &               0.134 &         0.326 &    0.007 &         0.038 &           0.470 &          0.162 &            0.087 \\
handle-press-side-v1 &            0.200 &      0.017 &                 0.120 &              -0.003 &         0.357 &   -0.036 &        -0.021 &           0.160 &          0.036 &            0.087 \\
peg-unplug-side-v1   &            0.108 &      0.037 &                 0.041 &               0.210 &         0.296 &   -0.071 &        -0.060 &           0.169 &         -0.010 &            0.085 \\
push-back-v1         &            0.145 &      0.011 &                 0.098 &               0.095 &         0.264 &    0.002 &        -0.066 &           0.311 &          0.063 &            0.087 \\
push-v1              &            0.170 &      0.074 &                 0.129 &               0.231 &         0.439 &   -0.003 &        -0.022 &           0.238 &          0.058 &            0.113 \\
push-wall-v1         &            0.115 &      0.047 &                 0.108 &               0.222 &         0.425 &   -0.009 &        -0.039 &           0.229 &          0.007 &            0.097 \\
shelf-place-v1       &            0.121 &      0.104 &                 0.098 &               0.028 &         0.110 &   -0.014 &        -0.009 &           0.323 &          0.097 &            0.089 \\
stick-pull-v1        &            0.162 &      0.070 &                 0.096 &               0.108 &         0.261 &    0.048 &         0.105 &           0.424 &          0.282 &            0.097 \\
window-close-v1      &            0.087 &     -0.036 &                 0.051 &               0.228 &         0.386 &   -0.005 &         0.034 &           0.337 &         -0.008 &            0.098 \\
\bottomrule
\end{tabular}

==> 609bc59dc39be977132478d8 copy/technical_details.tex <==
\subsection{Tasks details}
\label{sec:obs_act_rew}
\benchmark{} consists of a series of robotic tasks performed by a simulated Sawyer robot, each lasting for $200$ steps. Individual tasks come from \metaworld{}~\cite{metaworld} (benchmark released on MIT license) and as such, they have a significantly shared structure. This includes a common definition of the observation and action space as well as a similar reward structure.% \michal{Actually, the same reward structure, right?}
\paragraph{Observations} The observation space is $12$-dimensional, consisting of:
\begin{itemize}
    \item the $3$D Cartesian position of the robot end-effector ($3$ numbers),
    \item the $3$D Cartesian positions of one or two objects that the robot manipulates\footnotemark{} (6 numbers),
    \item the $3$D Cartesian position of the goal to be reached (3 numbers).
\end{itemize}
\footnotetext{For tasks with one object, the excessive coordinates are zeroed out.}
\paragraph{Actions} The action space is $4$-dimensional, including the requested $3$D end-effector position change and the gripper actuator delta. %\piotrm{someone verify please} \michal{I think this is ok.}

\paragraph{Rewards} \metaworld{} proposes a careful design of rewards, which ensures that tasks are solvable and exhibit shared structure across the tasks. These rewards are task-specific, see \cite[Section 4.2, Table 3]{metaworld} and are used only in training.


In the evaluation phase, a binary success metric is used
\begin{equation}
    \mathbb{I}_{{\| o-g \|}_{2}}< \varepsilon, \label{eq:evaluation_metric}
\end{equation}
where $o,g$ are the $3$D positions the object and goal, respectively, and  $\varepsilon$ is a task-specific threshold, see \cite[Table 4]{metaworld}.

\subsection{Sequences}\label{sec:sequences_appendix}
Our benchmark consists of two long CW10, \cwtwenty{} sequences and $8$ triples.

The CW10 sequence is: {\small \textsc{hammer-v1}, \textsc{push-wall-v1}, \textsc{faucet-close-v1}, \textsc{push-back-v1}, \textsc{stick-pull-v1},
\textsc{handle-press-side-v1}, \textsc{push-v1}, \textsc{shelf-place-v1}, \textsc{window-close-v1}, \textsc{peg-unplug-side-v1}}.

The \cwtwenty{} is CW10 repeated twice. The triples are presented in Section \ref{sec:triplets_appendix}.

\subsection{Training and evaluation details}\label{app:training_details}
We use an implementation of SAC algorithm \cite{DBLP:conf/icml/HaarnojaZAL18, DBLP:journals/corr/abs-1812-05905} based on \cite{SpinningUp2018} , which we ported to TensorFlow 2. SAC is an actor-critic type algorithm that uses neural networks in two different roles: the policy network (actor) and the value function network (critic).

Both the actor and critic are randomly initialized at the start of the first task and then are trained through the whole sequence, retaining parameters from previous tasks.

In all cases, except for A-GEM and Perfect Memory, we use CL algorithms only for the policy networks, for details see Section \ref{sec:critic_regularizaiton_appendix}.

\paragraph{Task handling} Each task is trained for $1$M steps. The replay buffer is emptied when a new task starts. For the first $10$K steps, actions are sampled uniformly from the action space. After these, actions are sampled using the current policy. We use a warm-up period of $1$K steps before training neural networks.

\paragraph{SAC training} We perform $50$ optimization steps per each $50$ interactions collected. To this end, we use the Adam optimizer \cite{DBLP:journals/corr/KingmaB14}. Its internal statistics are reset for each task. The maximum entropy coefficient $\alpha$ is tuned automatically \cite{DBLP:journals/corr/abs-1812-05905}, so that the average standard deviation of Gaussian policy matches the target value $\sigma_t =0.089$.

\paragraph{Policy evaluation} Performance on all tasks is measured (mean of \eqref{eq:evaluation_metric} on $10$ stochastic trajectories) every $20K$ steps. In the case of some metrics, we average over $5$ points in time to get smoother results.

% These evaluations are used to compute the following metrics: \maciejw{is something missing here?} for forward transfer, all the points are used; for average performance and forgetting last 5 points from each task are used (to smoothen the metrics).


\subsection{Network architecture}\label{sec:network_architecture_appendix}
We use a network with $4$ linear layers, each consisting of $256$ neurons. We add Layer Normalization \cite{DBLP:journals/corr/BaKH16} after the first layer. We use leaky ReLU activations (with $\alpha = 0.2$) after every layer except the first one, where we use the tanh activation, which is known to work well with Layer Normalization layers.

The network has as many heads as the corresponding sequence, e.g. $20$ for \cwtwenty{}. In Appendix~\ref{sec:onehot} we present experiments in which a single head is used, and the task id input is provided.


The presented architecture is used for both the actor and the critic. The actor network input consists of an observation, and it outputs the mean and log standard deviation of the Gaussian distribution on the action space. These outputs are produced for each task by its respective head. The critic network input consists of an observation and action, and it outputs a scalar value for each task head. %\piotrm{Do we have multiple heads for the critic? These are not needed in most cases (though not harmuful).} \michal{Yes, we use it}

% \piotrm{Write in little more details. I.e. say something about the value network and policy network.}


\subsection{Hyperparameters} \label{sec:hyperparameters_appendix}
We performed hyperparameter search in two stages. In the first stage, we selected hyperparameters of the SAC algorithm, which are common among all the methods. We measured the performance training on the \cwtwenty{} sequence using only the fine-tuning method. As the metric, we used the mean performance at the end of the training of each task. We present the search space and selected parameters in Table~\ref{hparams:general}.

%  First, we select the base hyperparameters that are common among all the methods, i.e.\ learning rate, batch size, discount factor $\gamma$ and target output standard deviation (see Appendix~\ref{app:training_details}). We perform the search by checking how respective settings perform with fine-tuning method. The criterion for selecting the best parameters is averaged performance, where for every task we take the performance at the end of learning of this task. This is because regular average performance for the final model is poor for the fine-tuning method no matter what parameters, and we want to select such a setting in which at least single-task learning is efficient.
In the second stage, we tuned method-specific hyperparameters using the final average performance as the objective. These are presented in Appendix~\ref{sec:cl_methods_appendix}.

\begin{table}
    \centering
    \begin{tabular}{ lcc }
        \toprule
        parameter                    & search space                                         & selected value \\
        \midrule
        learning rate                & $\{\num{3e-5}, \num{1e-4}, \num{3e-4}, \num{1e-3}\}$ & $\num{1e-3}$   \\
        batch size                   & $\{128, 256, 512\}$                                  & $128$          \\
        discount factor $\gamma$     & $\{0.95, 0.99, 0.995\}$                              & $0.99$         \\
        target output std $\sigma_t$ & $\{0.03, 0.089, 0.3\}$                               & $0.089$        \\
        replay buffer size           & ---                                                  & 1M             \\
        \bottomrule
    \end{tabular}
    \caption{Search space for the common hyperparameters.}
    \label{hparams:general}
\end{table}

\subsection{Bootstrap confidence intervals}\label{sec:confidence_intervals}
We use non-parametric bootstrap \cite{efron1994introduction} to calculate confidence intervals. Reinforcement learning typically has rather high variability. We found that using $20$ seeds usually results in informative intervals.

Unless specified otherwise, in all numerical results below, we use at least $20$ seeds and report $90\%$ confidence intervals.

\subsection{Infrastructure used} \label{sec:infrastructure_used} The typical configuration of a computational node used in our experiments was: the Intel Xeon E5-2697 $2.60$GHz processor with $128$GB memory. On a single node, we ran $3$ or $4$ experiments at the same time. A single experiment on the CW20 sequence takes about $100$ hours (with substantial variability with respect to the method used). We did not use GPUs; we found that with the relatively small size of the network, see Section \ref{sec:network_architecture_appendix} it offers only slight wall-time improvement while generating substantial additional costs. 

==> 609bc59dc39be977132478d8 copy/transfer_matrix.tex <==
In Table \ref{tab:app:transfer_matrix} we show the transfer matrix corresponding to Figure \ref{fig:transfer_matrix_haatmmap} (Section \ref{sec:task_sets}). Recall that the transfer matrix is aimed to measure the relationship between each two tasks 
(for transfer on  \cwtwenty{} see Table \ref{tab:transfer_table}). 
%
%Notice that there are only a few negative forward transfer cases, and those are of a rather small magnitude (perhaps  unsurprisingly, as the tasks are related). There are also visible patterns in the matrix. For instance, some tasks such as \textsc{peg-unplug-side-v1} or \textsc{push-back-v1} benefit from a relatively large forward transfer, (almost) irrespective of the first task. Furthermore, 
Most entries in the Table \ref{tab:app:transfer_matrix} are positive, however, some tasks seem to interfere with one another (most notably \textsc{peg-unplug-v1} (9) followed by \textsc{push-v1} (6)). Some of the factors influencing the transfer are: similarity in visual representation (e.g. objects on the scene), reward structure (reach, grasp, place), or direction in which the robotic arm moves. 
%
The average forward transfer given the second task (columns) is more variable than the corresponding quantity for the first task (rows), with the standard deviation equal to $0.21$ and $0.07$, respectively. %\kucil{let someone review this}

%\kucil{notice: place-shelf (7) and peg-unplug (9) as well also have rewards for reach, grasp and place, but perform so-so in the matrix.}

\begin{table}[h]
    \centering
\small
\rotatebox{90}{
\begin{tabular}{p{1.1cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}p{.9cm}|p{.6cm}}
\toprule
Second task &                    0 &                     1 &                  2 &                   3 &                    4 &                  5 &                     6 &                  7 &                  8 &                    9 & mean \\
First task &                      &                       &                    &                     &                      &                    &                       &                    &                    &                     & \\
\midrule
0          &    0.42 [0.32, 0.51] &    0.13 [-0.01, 0.24] &  0.64 [0.56, 0.70] &   0.58 [0.35, 0.76] &    0.24 [0.12, 0.35] &  0.48 [0.39, 0.56] &    0.03 [-0.09, 0.14] &  0.58 [0.54, 0.62] &  0.32 [0.26, 0.38] &    0.47 [0.05, 0.81]&0.39 \\
1          &    0.13 [0.01, 0.25] &   -0.05 [-0.18, 0.05] &  0.32 [0.11, 0.48] &   0.76 [0.72, 0.79] &   0.01 [-0.09, 0.11] &  0.46 [0.38, 0.53] &   -0.04 [-0.12, 0.04] &  0.28 [0.21, 0.35] &  0.36 [0.30, 0.42] &    0.78 [0.69, 0.85]&0.30 \\
2          &   0.04 [-0.08, 0.15] &   -0.04 [-0.10, 0.03] &  0.50 [0.35, 0.63] &   0.75 [0.72, 0.78] &   0.01 [-0.08, 0.10] &  0.26 [0.19, 0.33] &  -0.17 [-0.30, -0.06] &  0.32 [0.22, 0.41] &  0.27 [0.17, 0.35] &    0.79 [0.71, 0.85]&0.27 \\
3          &   0.03 [-0.22, 0.24] &  -0.15 [-0.30, -0.01] &  0.40 [0.14, 0.61] &   0.47 [0.23, 0.67] &   0.09 [-0.00, 0.18] &  0.42 [0.34, 0.49] &    0.01 [-0.10, 0.11] &  0.39 [0.29, 0.48] &  0.32 [0.24, 0.40] &   0.33 [-0.08, 0.66]&0.23 \\
4          &   0.19 [-0.02, 0.36] &     0.21 [0.14, 0.28] &  0.45 [0.20, 0.63] &   0.47 [0.22, 0.70] &    0.42 [0.34, 0.50] &  0.41 [0.32, 0.50] &     0.19 [0.11, 0.26] &  0.53 [0.46, 0.59] &  0.36 [0.28, 0.43] &   0.38 [-0.05, 0.71]&0.36 \\
5          &   0.05 [-0.08, 0.16] &   -0.00 [-0.14, 0.11] &  0.55 [0.43, 0.65] &   0.64 [0.49, 0.74] &   0.05 [-0.04, 0.13] &  0.51 [0.45, 0.56] &  -0.14 [-0.25, -0.05] &  0.20 [0.06, 0.33] &  0.32 [0.25, 0.38] &  -0.01 [-0.61, 0.50]&0.22 \\
6          &    0.20 [0.08, 0.31] &   -0.06 [-0.16, 0.03] &  0.47 [0.35, 0.57] &   0.78 [0.75, 0.81] &   0.09 [-0.03, 0.19] &  0.55 [0.50, 0.60] &   -0.01 [-0.08, 0.06] &  0.30 [0.18, 0.41] &  0.42 [0.35, 0.48] &    0.81 [0.77, 0.85]&0.36 \\
7          &    0.29 [0.09, 0.44] &   -0.03 [-0.14, 0.07] &  0.33 [0.07, 0.53] &  0.20 [-0.10, 0.47] &    0.14 [0.04, 0.24] &  0.42 [0.35, 0.48] &   -0.06 [-0.17, 0.05] &  0.40 [0.31, 0.49] &  0.33 [0.24, 0.41] &   0.10 [-0.48, 0.57]&0.21 \\
8          &  -0.10 [-0.33, 0.10] &     0.06 [0.00, 0.12] &  0.24 [0.04, 0.41] &   0.69 [0.63, 0.74] &  -0.01 [-0.11, 0.08] &  0.22 [0.15, 0.28] &   -0.02 [-0.08, 0.04] &  0.42 [0.34, 0.49] &  0.36 [0.29, 0.43] &    0.80 [0.75, 0.84]&0.27 \\
9          &   0.10 [-0.09, 0.26] &   -0.05 [-0.15, 0.04] &  0.30 [0.06, 0.48] &   0.53 [0.34, 0.68] &  -0.02 [-0.11, 0.08] &  0.18 [0.08, 0.26] &  -0.28 [-0.40, -0.16] &  0.21 [0.12, 0.30] &  0.31 [0.25, 0.37] &    0.74 [0.63, 0.83]&0.20 \\
\midrule
mean& 0.14&	0.00&	0.42	&0.59&	0.10&	0.39	&-0.05&	0.36	&0.34	&0.52& 0.28\\
\bottomrule
\end{tabular}}
    \caption{Transfer matrix. Normalized forward transfers for the second task. For task names see Section \ref{sec:sequences_appendix}.}
    \label{tab:app:transfer_matrix}
\end{table}

% \piotrm{Put some story}

\subsection{Diagonal transfers}\label{sec:diagonal_transfers_appendix}
The transfers on the diagonal (i.e., between the same tasks) are smaller than expected. We enumerate possible reasons: using multi-head architecture, buffer resetting, and uniform sampling exploration policy for the second task. These design elements are generally required when switching tasks, but not on the diagonal, where we resume the same task. This makes the diagonal of the transfer matrix suitable for an in-depth ablation analysis.


% In Table \ref{tab:diagonal_transfer} and example curves in in Figure \ref{fig:diagonal_appendix} we present results for four settings.
The experiments for the whole diagonal are summarized in Table \ref{tab:diagonal_transfer} and example curves are shown in Figure \ref{fig:diagonal_appendix}. We tested four settings. Multi Head (reset buffer) is our standard setting. Changing to a single head network, dubbed as Single Head (reset buffer), brings no significant difference. However, keeping the examples in the buffer in Single Head (no buffer reset) yields a major improvement. Similarly, in Single Head (no random exploration), when we do not perform random exploration at the task change the performance improves. We conjecture, that resetting the buffer and performing random exploration results in distributional shift, which is hard to be handled by SAC. %\piotrm{Verify please. Possilby we can also plug off-policy story.} \maciejw{Sounds good.}

% We found that resetting the buffer has the biggest impact on the performance of the second task (i.e., the one we transfer to). Using the multiple heads and random exploration is of smaller relevance. \maciejw{It is not exactly true that random exploration is of smaller relevance and I think we should explicitly say why we do not use it.}



\begin{table}\scriptsize
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        Task                 & MH (reset buffer) & SH (reset buffer) & SH (no buffer reset) & SH (no random exp) \\
        \midrule
        \texttt{hammer-v1}            & 0.42              & 0.26              & 0.56                 & 0.74               \\
        \texttt{push-wall-v1}         & -0.05             & 0.06              & 0.55                 & 0.40               \\
        \texttt{faucet-close-v1}      & 0.50              & 0.64              & 0.60                 & 0.78               \\
        \texttt{push-back-v1}         & 0.47              & 0.41              & 0.67                 & 0.68               \\
        \texttt{stick-pull-v1}        & 0.42              & 0.37              & 0.60                 & 0.63               \\
        \texttt{handle-press-side-v1} & 0.51              & 0.53              & 0.53                 & 0.68               \\
        \texttt{push-v1}              & -0.01             & -0.03             & 0.64                 & 0.35               \\
        \texttt{shelf-place-v1}       & 0.40              & 0.23              & 0.29                 & 0.40               \\
        \texttt{window-close-v1}      & 0.36              & 0.50              & 0.45                 & 0.52               \\
        \texttt{peg-unplug-side-v1}   & 0.74              & 0.83              & 0.97                 & 0.96               \\
        \midrule
        mean              & 0.38              & 0.38              & 0.58                 & 0.61               \\
        \bottomrule
    \end{tabular}
    \caption{Transfers on the diagonal. MH and SH stand for multi-head and single-head, respectively.}\label{tab:diagonal_transfer}
\end{table}



\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/appendix/diagonal.png}
    \caption{Success rates for example tasks on the diagonal of the transfer matrix. The blue line is the standard setup. Note, that its poor performance in the first part of each plot is expected, as we evaluate the head which has not yet been trained. Performance improves when we keep the samples in the buffer when switching the task or when we disable the exploration through uniform policy.}
    \label{fig:diagonal_appendix}
\end{figure}

% \begin{itemize}
%     % \item The transfers on the diagonal are not very high, sometimes they are even slightly negative (push-wall-v1 (id 1) = -0.05, push-v1 (id 6) = -0.01). Why is that?
%     \item We examine whether switching form multi-head (blue lines) to single-head (orange line) helps. It sometimes helps, but there is still a significant "collapse" at the point when we change task.
%     % \item We then test what happens if we do not reset the buffer samples (green line). There is no collapse, forward transfer is much higher. This is cheating in some sense - this approach is incompatible with the CL mindset of not having samples from the previous task and would not work outside the diagonal (reservoir sampling fails in our regular experiments).
%     \item In SAC if we do not have any samples in the buffer, we use uniform sampling, let's use our standard policy (red line) instead. This works better then orange line but sometimes worse than green line. This would hinder exploration outside the diagonal.
%     \item Third plot is especially interesting - seems like dropping old samples actually helps here (red line higher than green line).
% \end{itemize}

==> 609bc59dc39be977132478d8 copy/triplets.tex <==
In addition to the CW10 and CW20 sequences, we propose eight triplets. They are sequences of three tasks aimed to allow rapid experimenting. The triplets were selected in order to capture situations when remembering is crucial for forward transfer. That is, we consider tasks $A \rightarrow B \rightarrow C$, where $A \rightarrow C$ exhibits bigger forward transfer than $B \rightarrow C$ (based on the transfer matrix), see Table \ref{tab:triplet_transfers} . We propose the following triplets:

\begin{enumerate}
    \item  $\texttt{push-v1}\rightarrow \texttt{window-close-v1} \rightarrow \texttt{hammer-v1}$
    \item  $\texttt{hammer-v1} \rightarrow \texttt{window-close-v1} \rightarrow \texttt{faucet-close-v1} $
    \item  $\texttt{stick-pull-v1} \rightarrow \texttt{push-back-v1} \rightarrow \texttt{push-wall-v1} $
    \item  $\texttt{push-wall-v1} \rightarrow \texttt{shelf-place-v1} \rightarrow \texttt{push-back-v1}$
    \item  $\texttt{faucet-close-v1} \rightarrow \texttt{shelf-place-v1} \rightarrow \texttt{push-back-v1}$
    \item  $\texttt{stick-pull-v1} \rightarrow \texttt{peg-unplug-side-v1} \rightarrow \texttt{stick-pull-v1}$
    \item  $\texttt{window-close-v1} \rightarrow \texttt{handle-press-side-v1} \rightarrow \texttt{peg-unplug-side-v1}$
    \item  $\texttt{faucet-close-v1} \rightarrow \texttt{shelf-place-v1} \rightarrow \texttt{peg-unplug-side-v1}$
\end{enumerate}

In Figure \ref{fig:more_triples_appendix} and Table \ref{tab:triplet_transfers} we present evaluations for the third task. On most of the triplets, the tested methods  (Fine-tuning, EWC, PackNet, Perfect Memory) are not able to reach the performance obtained by direct transfer $A \rightarrow C$. Moreover, Fine-tuning often outperforms the rest of the methods. Interestingly, in triplets 7 and 8, Fine-tuning is able to achieve transfer comparable to $A \rightarrow C$, while EWC and PackNet smaller one similar to $B \rightarrow C$. Perfect memory does not perform well on any triplet, which is consistent with our experiments on the long sequences.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/appendix/triplets.png}
    \caption{Performance of selected methods on the triplets sequences.}
    \label{fig:more_triples_appendix}
\end{figure}

\begin{table}
    \centering\scriptsize
    \begin{tabular}{lp{1cm}p{1cm}p{2cm}p{2cm}p{2cm}p{2.3cm}}
        \toprule
        Triplet & A$\rightarrow$ C & B $\rightarrow$ C & A $\rightarrow$ B $\rightarrow$ C (Fine-tuning) & A $\rightarrow$ B $\rightarrow$ C (PackNet) & A $\rightarrow$ B $\rightarrow$ C (EWC) & A $\rightarrow$ B $\rightarrow$ C (Perfect Mem.) \\
        \midrule
        1       & 0.20             & -0.10             & -0.14                                           & -0.21                                       & -0.50                                   & -1.73                                            \\
        2       & 0.64             & 0.24              & 0.06                                            & 0.36                                        & 0.20                                    & -0.98                                            \\
        3       & 0.21             & -0.15             & 0.10                                            & 0.28                                        & -0.31                                   & -1.09                                            \\
        4       & 0.76             & 0.20              & 0.76                                            & 0.56                                        & 0.62                                    & -0.52                                            \\
        5       & 0.75             & 0.20              & 0.76                                            & 0.20                                        & 0.22                                    & -0.64                                            \\
        6       & 0.42             & -0.02             & 0.14                                            & 0.10                                        & 0.29                                    & -0.49                                            \\
        7       & 0.80             & -0.01             & 0.79                                            & 0.11                                        & 0.06                                    & -0.00                                            \\
        8       & 0.79             & 0.10              & 0.74                                            & 0.15                                        & 0.05                                    & -0.46                                            \\
        \midrule
        mean    & 0.57             & 0.06              & 0.40                                            & 0.19                                        & 0.08                                    & -0.74                                            \\
        \bottomrule
    \end{tabular}
    \caption{Forward Transfers for triplets.}\label{tab:triplet_transfers}
\end{table}

==> experiments_old_28_01.tex <==

Main experimental takeaways discussion
\begin{itemize}
    \item Forgetting seems mainly to be mitigated by existing methods.
    \item Methods tend to transfer poorly - lack of transfer between tasks seems embarrassing to the field.
    \item Methods saturate on longer sequences.
\end{itemize}

\maciejw{I wonder if these takeaways aren't too much connected to the hyperparameters we have chosen. For example, if we used smaller regularization coefficient for EWC then it would have better transfer and more forgetting. On the other hand, we chose these hyperparameters by looking at the thing that most people look at in CL - the average performance at the end of the training. So maybe we could argue that focusing on that in some sense discourages people from caring about forward transfer? 2021-01-27}

In our experiments, we pose the following research questions: what is the level of the forward transfer and forgetting in robotic tasks without using CL methods? How do CL methods change this picture? More specifically, is forgetting helpful or harmful for forward transfer? Further, we ask how much information about pairs and triples could be beneficial for longer sequences.

\piotrm{We should state take-aways and also put them in the intro.}


\subsection{\benchmark{} experiments}
Ideas:
\begin{enumerate}
    \item Present value at the end of ten tasks (i.e. the right most one on Figure \ref{fig:training_graph}) as on of main matric.
    \item Have it for all CL methods.
    \item Present value at the end of twenty tasks as the second main metric.
    \item Calculate forgetting -- \razp{I'm ashamed to say I'm not even sure what people tend to report usually. I tend to only look at learning curves and make "qualitative" observations. I think Arslan had proposed something on one of his paper that seemed relatively popular; but I think is exactly point (1) which is the performance at the end on all previous tasks. I think in progressive nets paper we had a nice table where we colored with green vs blue and basically was looking at the performance of training each task ? or was it some AUC as well. Someone should open that paper :) }(is it the classical thing to do?).
\end{enumerate}

\subsection{Pair experiments}
Ideas:

\begin{enumerate}
    \item Present the forward transfer matrices. Here probably a subset in the appendix the whole table
    \item Describe some stories behind:  various relations, @PM mockup
    \item Why we do not say anything about forgetting here? nice-to-have \razp{ There are some thoughts here. re: catastrophic forgetting. We will be measuring it. Would be nice to plot catastrophic forgetting vs forward transfer to see if there is some structure there (with respect to methods). The other thing is recovering of the forgotten policies. So if we have the sequence of 20 tasks where we revisit tasks. It would be nice here to see if there is a correlation between how much you remember the previous task and how quickly you recover it. }
    \item upper-bound
          \kucil{2021-01-22: transfer with significance correction. Also in the Appendix table with CIs}
\end{enumerate}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/heatmap_transfer.png}}%pair_plot_mockup.png}}
        \caption{\piotrm{todo please put the final version with desscription.} }\label{fig:transfer_matrix_haatmmap}
    \end{center}
    \vskip -0.2in
\end{figure}

% \begin{figure}[ht]
%     \vskip 0.2in
%     \begin{center}
%     \centerline{\includegraphics[width=\columnwidth]{imgs/transfer_heatmap_significant.png}}%pair_plot_mockup.png}}
%     \caption{fillme (significance correction). atm for comparison. (todo: put normalized)}
%     \end{center}
%     \vskip -0.2in
% \end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \subfigure[A $\rightarrow$ B $\rightarrow$ C]{
            \includegraphics[width=0.47\columnwidth]{imgs/triple.png}
        }
        \subfigure[A $\rightarrow$ B $\rightarrow$ A]{
            \includegraphics[width=0.47\columnwidth]{imgs/triple_to_self.png}
        }
        \caption{\textbf{How forgetting impacts the forward transfer.} Figures present performance on task C with different types of pretraining. (a) A $\rightarrow$ C has very positive transfer, but putting a destructive task B between them causes the model to forget useful knowledge from task A. (b) This effect appears even if we consider transfers to itself, i.e A $\rightarrow$ B $\rightarrow$ A.}
    \end{center}
    \vskip -0.2in
\end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/positive_transfer_graph_example.png}}
        \caption{\textbf{Cherry pick with positive transfer}.}
    \end{center}
    \vskip -0.2in
\end{figure}

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{imgs/negative_transfer_example.png}}
        \caption{\textbf{Cherry pick with negative transfer transfer}.}
    \end{center}
    \vskip -0.2in
\end{figure}

Detailed tables and graphs are presented in Section \ref{sec:pair_experiments_appendix}.

\subsection{Triples experiments}

\begin{itemize}
    \item Possibly run progressive nets as baseline.
\end{itemize}

\section{Random observations/notes}
\begin{itemize}
    \item \maciejw{Many algorithms didn't work as it is (e.g. EWC required deriving Fisher with some non-obvious assumptions). I know that RL aspects are not really our focus, but maybe we could have a paragraph somewhere where we say that there were some issues and refer the reader to the appendix for details?} This is RL specific.
    \item \maciejw{Continual learning methods perform much better when they do not regularize the critic, on the other hand it may be difficult to use them for retraining.}
    \item \maciejw{Experience replay methods, although they excel in supervised setting, do not perform very well in our benchmark. It maybe partly because they are forced to regularize the critic as well as the actor.}
    \item \maciejw{It seems that transfer from a task to itself is usually not as good as we would expect -- maybe because there is too much noise at the beginning of the training?}
    \item \michal{when we consider CL methods, transfer is diminished compared to vanilla, EXCEPT FOR PackNet. TODO: compare to "upper bound"}

    \item \michal{when the sequence of tasks is repeated, performance is surprisingly poor on second half - why?}
    \item \michal{Regarding poor "transfer" from X to X: at some point we observed that even just resetting the buffer after first "instance" of the same task leads to poor transfer metric. We'd need to double-check though}

    \item \piotrm{We observe little forgetting for any method but vanilla. See Figure \ref{fig:forgetting}} Than it would follow that methods are better because of transfers?
    \item \piotrm{We possibly need to justify the selection of $1$M steps more carefully, as the curves are still growing. See Figure \ref{fig:long_sequence}}
    \item \michal{In the current version (task set), MTL performs at the level of EWC and worse than PackNet -- should we worry?}
\end{itemize}

To do list:
\begin{itemize}
    \item For above see if there are some correlations @all
\end{itemize}
To do list (nice to have):
\begin{itemize}
    \item Multi-task learning with separate critics
    \item Find examples of backward transfer
    \item Run experiment without multi-head (possibly with task\_id instead)
    \item Put a case study forgetting vs transfer (e.g. "L2 hps analysis" done by Maciek)
    \item Possibly mention (or compute if relevant) 'transfer score' of progressive nets.
\end{itemize}

==> forgetting_qualitiatie_analysis.tex <==
\subsubsection{Vanilla and AGEM} The forgetting occurs quickly after the training of a given task has finished, see Figure \ref{fig:forgetting_agem} for AGEM, results for the vanilla method are similar. 


\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=agem_pm_zeroed.png}}
    \caption{Forgetting plot for AGEM (we zero the plot until the task ends)} \label{fig:forgetting_agem}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{EWC} For EWC the forgetting is rather small with the exception of the first task, which decreases quickly after its training has completed, see Figure \ref{fig:forgetting_ewc}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=ewc_pm_zeroed.png}}
    \caption{Forgetting plot for EWC (we zero the plot until the task ends)} \label{fig:forgetting_ewc}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{MAS} MAS experiences mild forgetting shortly after a given task has completed, see Figure \ref{fig:forgetting_mas}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=mas_pm_zeroed.png}}
    \caption{Forgetting plot for MAS (we zero the plot until the task ends)} \label{fig:forgetting_mas}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{Packnet} See Figure \ref{fig:forgetting_packnet} (note that some variations are due to noise).
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=packnet_pm_zeroed.png}}
    \caption{Forgetting plot for packnet (we zero the plot until the task ends)} \label{fig:forgetting_packnet}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{VCL} VCL behaves relatively worse than other methods. We can observe small decrease over the whole training, see Figure \ref{fig:forgetting_vlc}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=vcl_pm_zeroed.png}}
    \caption{Forgetting plot for VCL (we zero the plot until the task ends)} \label{fig:forgetting_vlc}
    \end{center}
    \vskip -0.2in
\end{figure*}

\subsubsection{L2} L2 is surprisingly good taking into account it simplicity. We observe, however, an erratic drops in performace in a 'random' moments. We conjecture that these are when conflicting information appears. See Figure \ref{fig:forgetting_l2}.
\begin{figure*}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{imgs/plot_individualcl_method=l2_pm_zeroed.png}}
    \caption{Forgetting plot for L2 (we zero the plot until the task ends)} \label{fig:forgetting_l2}
    \end{center}
    \vskip -0.2in
\end{figure*}

==> forgetting_table.tex <==
\begin{table}[h!]
    \begin{center}
        \begin{tabular}{lrrrrrrrrrr}
            \toprule
            {} &  \rotatebox[origin=c]{90}{hammer-v1} &  \rotatebox[origin=c]{90}{push-wall-v1} &  \rotatebox[origin=c]{90}{faucet-close-v1} &  \rotatebox[origin=c]{90}{push-back-v1} &  \rotatebox[origin=c]{90}{stick-pull-v1} &  \rotatebox[origin=c]{90}{handle-press-side-v1} &  \rotatebox[origin=c]{90}{push-v1} &  \rotatebox[origin=c]{90}{shelf-place-v1} &  \rotatebox[origin=c]{90}{window-close-v1} &  \rotatebox[origin=c]{90}{peg-unplug-side-v1} \\
            cl\_method &                                      &                                         &                                            &                                         &                                          &                                                 &                                    &                                           &                                            &                                               \\
            \midrule
            None      &                                 0.89 &                                    0.72 &                                       0.95 &                                    0.99 &                                     0.68 &                                            0.96 &                               0.83 &                                      0.45 &                                       0.82 &                                          0.00 \\
            agem      &                                 0.88 &                                    0.72 &                                       0.86 &                                    0.90 &                                     0.75 &                                            0.86 &                               0.78 &                                      0.84 &                                       0.76 &                                          0.00 \\
            ewc       &                                 0.38 &                                    0.13 &                                       0.05 &                                    0.03 &                                    -0.11 &                                           -0.06 &                              -0.01 &                                     -0.00 &                                       0.02 &                                          0.00 \\
            l2        &                                 0.14 &                                    0.06 &                                       0.14 &                                    0.00 &                                    -0.02 &                                            0.01 &                               0.05 &                                     -0.01 &                                      -0.02 &                                          0.00 \\
            mas       &                                 0.01 &                                    0.03 &                                       0.05 &                                   -0.02 &                                    -0.14 &                                           -0.08 &                              -0.00 &                                      0.02 &                                      -0.01 &                                          0.00 \\
            packnet   &                                -0.07 &                                    0.07 &                                       0.00 &                                    0.00 &                                    -0.00 &                                            0.00 &                               0.04 &                                     -0.00 &                                      -0.03 &                                          0.00 \\
            vcl       &                                 0.17 &                                    0.15 &                                       0.20 &                                    0.15 &                                     0.09 &                                            0.43 &                               0.11 &                                      0.07 &                                       0.13 &                                          0.00 \\
            \bottomrule
        \end{tabular}
        
        \caption{Averages over forgetting.} \label{tab:forgetting_table}
    \end{center}
\end{table}

==> long_transfer_tables.tex <==
\begin{table}
\centering
\caption{Summary of FT experiments}
\begin{tabular}{lllllll}
\toprule
identifier &                    FT &          FT\_first\_ten &         FT\_second\_ten &         Normalized FT & Normalized FT\_first\_ten & CI\_second\_half\_normalized\_ft \\
\midrule
      None &     0.07 [0.06, 0.09] &     0.12 [0.11, 0.14] &     0.03 [0.00, 0.05] &     0.20 [0.17, 0.23] &       0.32 [0.29, 0.35] &            0.08 [0.04, 0.13] \\
       ewc &  -0.07 [-0.09, -0.05] &    0.01 [-0.02, 0.03] &  -0.14 [-0.17, -0.11] &  -0.19 [-0.25, -0.13] &      0.02 [-0.05, 0.07] &         -0.39 [-0.49, -0.30] \\
        l2 &  -0.25 [-0.29, -0.22] &  -0.21 [-0.25, -0.17] &  -0.30 [-0.33, -0.27] &  -0.75 [-0.87, -0.64] &    -0.64 [-0.77, -0.52] &         -0.86 [-0.97, -0.75] \\
       mas &  -0.19 [-0.20, -0.17] &  -0.13 [-0.15, -0.11] &  -0.24 [-0.27, -0.22] &  -0.52 [-0.58, -0.47] &    -0.36 [-0.42, -0.30] &         -0.68 [-0.77, -0.61] \\
   packnet &     0.07 [0.06, 0.09] &     0.10 [0.08, 0.11] &     0.05 [0.03, 0.07] &     0.18 [0.14, 0.22] &       0.22 [0.17, 0.27] &            0.14 [0.09, 0.19] \\
\bottomrule
\end{tabular}\label{tab:long_forward_transfer_table}
\end{table}

%\begin{table}
%\centering
%\caption{Summary of FT experiments}
%\label{tab:long_forward_transfer_table}
%\begin{tabular}{lrrrrrr}
%\toprule
%identifier &    FT &  FT\_first\_ten &  FT\_second\_ten &  Normalized FT &  Normalized FT\_first\_ten &  Normalized FT\_second\_ten \\
%\midrule
%      None &  0.08 &          0.13 &           0.04 &           0.22 &                     0.33 &                      0.10 \\
%       ewc & -0.05 &          0.02 &          -0.13 &          -0.13 &                     0.08 &                     -0.33 \\
%        l2 & -0.23 &         -0.20 &          -0.27 &          -0.69 &                    -0.61 &                     -0.77 \\
%       mas & -0.18 &         -0.13 &          -0.22 &          -0.49 &                    -0.36 &                     -0.62 \\
%   packnet &  0.04 &          0.16 &          -0.08 &           0.05 &                     0.38 &                     -0.28 \\
%\bottomrule
%\end{tabular}
%\end{table}


\begin{table}[ht]
\centering
\caption{Normalized Forward Transfer, first ten tasks}
\begin{tabular}{lllllllllll}
\toprule
train/active\_env &                     0 &                     1 &                    2 &                     3 &                     4 &                     5 &                     6 &                     7 &                     8 &                     9 \\
identifier &                       &                       &                      &                       &                       &                       &                       &                       &                       &                       \\
\midrule
None       &     0.13 [0.05, 0.20] &    0.06 [-0.08, 0.19] &    0.39 [0.24, 0.51] &     0.76 [0.73, 0.79] &    0.08 [-0.05, 0.20] &     0.55 [0.50, 0.59] &   -0.11 [-0.24, 0.01] &     0.13 [0.04, 0.22] &     0.44 [0.38, 0.50] &     0.77 [0.70, 0.81] \\
ewc        &     0.13 [0.05, 0.20] &  -0.10 [-0.19, -0.02] &    0.35 [0.20, 0.49] &     0.66 [0.51, 0.76] &  -0.36 [-0.45, -0.27] &     0.14 [0.03, 0.25] &  -0.81 [-0.98, -0.63] &  -0.10 [-0.19, -0.01] &     0.35 [0.22, 0.47] &   -0.11 [-0.63, 0.32] \\
l2         &     0.14 [0.07, 0.21] &  -0.39 [-0.52, -0.25] &  -0.09 [-0.40, 0.20] &  -0.26 [-0.52, -0.01] &  -0.45 [-0.52, -0.39] &  -1.84 [-2.42, -1.28] &  -1.69 [-1.93, -1.44] &  -0.20 [-0.26, -0.15] &  -0.91 [-1.46, -0.37] &  -0.68 [-1.21, -0.25] \\
mas        &     0.13 [0.05, 0.20] &  -0.63 [-0.72, -0.53] &   0.04 [-0.20, 0.24] &   -0.09 [-0.31, 0.12] &  -0.35 [-0.45, -0.25] &  -0.44 [-0.59, -0.30] &  -1.38 [-1.60, -1.17] &  -0.18 [-0.25, -0.12] &   -0.18 [-0.56, 0.14] &  -0.51 [-1.06, -0.04] \\
packnet    &  -0.49 [-0.65, -0.35] &   -0.08 [-0.19, 0.02] &    0.33 [0.09, 0.50] &     0.80 [0.76, 0.83] &  -0.21 [-0.33, -0.09] &    0.05 [-0.22, 0.29] &     0.12 [0.04, 0.20] &     0.44 [0.34, 0.53] &     0.45 [0.28, 0.58] &     0.80 [0.72, 0.86] \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[ht]
\centering
\caption{Normalized Forward Transfer, second ten tasks}
\begin{tabular}{lllllllllll}
\toprule
train/active\_env &                    10 &                    11 &                    12 &                    13 &                    14 &                    15 &                    16 &                    17 &                    18 &                    19 \\
identifier &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       \\
\midrule
None       &   -0.30 [-0.62, 0.00] &  -0.21 [-0.30, -0.12] &    0.04 [-0.13, 0.20] &     0.53 [0.44, 0.60] &  -0.19 [-0.31, -0.05] &     0.48 [0.41, 0.56] &  -0.79 [-0.96, -0.63] &    0.02 [-0.07, 0.11] &     0.52 [0.45, 0.59] &     0.73 [0.66, 0.78] \\
ewc        &  -0.66 [-0.97, -0.37] &  -0.57 [-0.70, -0.45] &  -0.36 [-0.67, -0.07] &     0.39 [0.25, 0.51] &  -0.47 [-0.53, -0.41] &    0.03 [-0.13, 0.19] &  -1.83 [-2.06, -1.60] &  -0.20 [-0.27, -0.13] &   -0.06 [-0.45, 0.28] &   -0.16 [-0.72, 0.29] \\
l2         &  -0.49 [-0.82, -0.16] &  -0.77 [-0.90, -0.65] &  -0.74 [-1.11, -0.42] &  -0.59 [-0.79, -0.41] &  -0.49 [-0.55, -0.43] &  -1.52 [-1.99, -1.08] &  -2.44 [-2.64, -2.25] &  -0.23 [-0.29, -0.18] &  -0.74 [-1.21, -0.29] &  -0.59 [-1.09, -0.18] \\
mas        &  -0.41 [-0.76, -0.09] &  -0.71 [-0.81, -0.61] &  -0.67 [-1.00, -0.38] &  -0.33 [-0.55, -0.13] &  -0.45 [-0.53, -0.37] &  -1.05 [-1.40, -0.72] &  -2.07 [-2.29, -1.85] &  -0.22 [-0.28, -0.17] &  -0.67 [-1.18, -0.18] &   -0.26 [-0.73, 0.14] \\
packnet    &  -0.41 [-0.74, -0.10] &    0.08 [-0.02, 0.17] &     0.42 [0.31, 0.50] &     0.82 [0.79, 0.85] &  -0.24 [-0.35, -0.13] &    0.17 [-0.00, 0.34] &  -0.34 [-0.47, -0.19] &   -0.03 [-0.12, 0.06] &     0.44 [0.28, 0.58] &     0.46 [0.14, 0.70] \\
\bottomrule
\end{tabular}
\end{table}



%\begin{table}[ht]
%\centering
%\caption{Normalized Forward Transfer, first ten tasks}
%\begin{tabular}{lp{1.5cm}rrrrrrrrr}
%\toprule
%train/active\_env &     0 &     1 &     2 &     3 &     4 &     5 &     6 &     7 &     8 &     9 \\
%identifier &       &       &       &       &       &       &       &       &       &       \\
%\midrule
%None       &  0.13 [0.11, 0.12] &  0.06 &  0.46 &  0.77 &  0.09 &  0.58 & -0.05 &  0.08 &  0.47 &  0.77 \\
%ewc        &  0.13 & -0.02 &  0.44 &  0.53 & -0.32 &  0.15 & -0.93 & -0.10 &  0.40 &  0.48 \\
%l2         &  0.11 & -0.30 &  0.00 & -0.23 & -0.43 & -1.68 & -1.82 & -0.19 & -0.64 & -0.87 \\
%mas        &  0.13 & -0.60 &  0.23 & -0.12 & -0.34 & -0.53 & -1.40 & -0.19 & -0.10 & -0.68 \\
%packnet    & -0.14 &  0.17 &  0.59 &  0.84 &  0.04 &  0.56 &  0.06 &  0.36 &  0.57 &  0.81 \\
%\bottomrule
%\end{tabular}
%\end{table}
%
%\begin{table}[ht]
%\centering
%\caption{Normalized Forward Transfer, second ten tasks}
%\begin{tabular}{lrrrrrrrrrr}
%\toprule
%train/active\_env &    10 &    11 &    12 &    13 &    14 &    15 &    16 &    17 &    18 &    19 \\
%identifier &       &       &       &       &       &       &       &       &       &       \\
%\midrule
%None       & -0.36 & -0.17 &  0.06 &  0.55 & -0.16 &  0.46 & -0.72 &  0.13 &  0.55 &  0.71 \\
%ewc        & -0.80 & -0.57 & -0.36 &  0.38 & -0.49 &  0.09 & -1.94 & -0.15 &  0.27 &  0.27 \\
%l2         & -0.31 & -0.87 & -0.62 & -0.41 & -0.49 & -1.15 & -2.62 & -0.23 & -0.75 & -0.29 \\
%mas        & -0.40 & -0.65 & -0.74 & -0.24 & -0.42 & -0.79 & -2.21 & -0.21 & -0.34 & -0.19 \\
%packnet    & -0.11 & -0.07 &  0.26 &  0.69 & -0.40 &  0.09 & -0.64 & -0.18 & -0.18 & -2.27 \\
%\bottomrule
%\end{tabular}
%\end{table}

==> pairs_vanilla_table.tex <==
\textbf{PM: this is now 15.01 a mock-up}

\begin{tabular}{lrrrrrrrrrr}
\toprule
task &  \rotatebox[origin=c]{90}{faucet-close-v1} &  \rotatebox[origin=c]{90}{hammer-v1} &  \rotatebox[origin=c]{90}{handle-press-side-v1} &  \rotatebox[origin=c]{90}{peg-unplug-side-v1} &  \rotatebox[origin=c]{90}{push-back-v1} &  \rotatebox[origin=c]{90}{push-v1} &  \rotatebox[origin=c]{90}{push-wall-v1} &  \rotatebox[origin=c]{90}{shelf-place-v1} &  \rotatebox[origin=c]{90}{stick-pull-v1} &  \rotatebox[origin=c]{90}{window-close-v1} \\
first\_task           &                  &            &                       &                     &               &          &               &                 &                &                  \\
\midrule
faucet-close-v1      &            0.182 &      0.015 &                 0.061 &               0.224 &         0.421 &   -0.043 &        -0.012 &           0.257 &          0.007 &            0.072 \\
hammer-v1            &            0.230 &      0.154 &                 0.112 &               0.134 &         0.326 &    0.007 &         0.038 &           0.470 &          0.162 &            0.087 \\
handle-press-side-v1 &            0.200 &      0.017 &                 0.120 &              -0.003 &         0.357 &   -0.036 &        -0.021 &           0.160 &          0.036 &            0.087 \\
peg-unplug-side-v1   &            0.108 &      0.037 &                 0.041 &               0.210 &         0.296 &   -0.071 &        -0.060 &           0.169 &         -0.010 &            0.085 \\
push-back-v1         &            0.145 &      0.011 &                 0.098 &               0.095 &         0.264 &    0.002 &        -0.066 &           0.311 &          0.063 &            0.087 \\
push-v1              &            0.170 &      0.074 &                 0.129 &               0.231 &         0.439 &   -0.003 &        -0.022 &           0.238 &          0.058 &            0.113 \\
push-wall-v1         &            0.115 &      0.047 &                 0.108 &               0.222 &         0.425 &   -0.009 &        -0.039 &           0.229 &          0.007 &            0.097 \\
shelf-place-v1       &            0.121 &      0.104 &                 0.098 &               0.028 &         0.110 &   -0.014 &        -0.009 &           0.323 &          0.097 &            0.089 \\
stick-pull-v1        &            0.162 &      0.070 &                 0.096 &               0.108 &         0.261 &    0.048 &         0.105 &           0.424 &          0.282 &            0.097 \\
window-close-v1      &            0.087 &     -0.036 &                 0.051 &               0.228 &         0.386 &   -0.005 &         0.034 &           0.337 &         -0.008 &            0.098 \\
\bottomrule
\end{tabular}
